Markovian Search with Ex-Ante Constraints: Theory and Applications to Socially Aware Algorithmic Hiring

We develop an algorithmic framework to incorporate "ex-ante" constraints on outcomes (that hold only on average) into stateful sequential search with costly inspection. Our framework encompasses the classical Weitzman's Pandora's box [Weitzman, 1979] as well as its extensions to joint Markovian scheduling [Dumitriu et al., 2003; Gittins, 1979], modeling richer processes such as multistage search with multiple layers of inspection. Ex-ante constraints in search are particularly motivated by social considerations in algorithmic hiring, where they adjust outcome distributions to promote equity and access. Building on the optimality of index-based policies in the unconstrained problems, we show that optimal policies under a single ex-ante constraint (e.g., demographic parity) retain an index-based structure but require (i) dual-based adjustments of the indices and (ii) randomization between two such adjustments via a "tie-breaking rule," both easy to compute and economically interpretable. We then extend our results to handle multiple affine constraints by reduction to a variant of the exact Carath\'eodory problem and providing a polynomial-time algorithm to construct an optimal randomized dual-adjusted index-based policy that satisfies all constraints simultaneously. For general affine and convex constraints, we develop a primal-dual algorithm that randomizes over a polynomial number of dual-based adjustments, yielding a near-feasible, near-optimal policy. All these results rely on the key observation that a suitable relaxation of the Lagrange dual function for these constrained problems admits index-based policies akin to those in the unconstrained setting. Finally, through a numerical study, we investigate the implications of various socially aware ex-ante constraints on the utilitarian loss (price of fairness), and examine whether they achieve their intended socially desirable outcomes.

==> tex/JMS-unconstrained.tex <==
\subsection{Optimal Policy for JMS with Arbitrary Rewards: Review and Refinement}
\label{sec:optimal-JMS-arbitrary}
The first step in solving \eqref{eq:opt-fair} is solving the same problem with no ex-ante constraints, that is, finding a policy $\policy$ that maximizes $\expect{\reward_\policy}$. Importantly, we allow the rewards $\vecreward=[R_i(s)]_{i\in[\altnum],s\in\states_i}$  to take negative or positive rewards in the JMS instance, which proves to be crucial for incorporating ex-ante constraints, as we have already seen in \Cref{sec:pandora} and we will also see later when we define dual-adjusted rewards (\Cref{sec:RAI}) for JMS.  We sketch how to devise a polynomial-time algorithm for this problem, even in such an instance.

% , as any solution to the following stochastic online program:
%  \begin{equation}
%  \label{eq:opt-unfair}
% \tag{\textsc{OPT-UNFAIR}}
%  \begin{aligned}
%  \OptUNFair\triangleq & \quad \max_{\policy\in\PolicySpace} ~~\expect{\reward_\policy} & 
%  \end{aligned}
% \end{equation}


Past work studying the JMS problem with linear rewards characterize the optimal policy by either assuming negative rewards (i.e., costs) for intermediate states and only allowing positive rewards for the terminal states (see, e.g.,  \cite{dumitriu2003playing,gupta2019markovian}), or considering the more general so called \emph{No Free Lunch (NFL)} assumption on the state-reward structure of the Markov chains (see, e.g., \cite{gittins1979bandit,kleinberg2017tutorial}) and showing a similar analysis extends.

\begin{definition}[\textbf{NFL \citep{kleinberg2017tutorial}}]
\label{def:NFL}
An alternative $\MC$ satisfies NFL if for any state $s\in\states$ with $\reward(s)>0$, there exists a terminal state $t\in\terminals$ such that $\transition(s,t)>0$.
\end{definition}
Under NFL assumption, the earlier work established the optimality of the \emph{Gittins index policy}~\citep{gittins1979bandit,dumitriu2003playing}, which is a generalization of the optimal index-based policy of \citeauthor{weitzman1979optimal} for the Pandora's box problem: Given an instance $\left\{\MC_i\right\}_{i\in[\altnum]}$, there exists an index mapping $\sigma:\cup_{i\in[\altnum]}\states_i\rightarrow \mathbb{R}$ such that choosing the Markov chain $\MC_i$ with maximum $\reserve_i(s_i)$ to inspect given states $\{s_i\}_{i\in[\altnum]}$ at each time, until either $\capacity$ number of the Markov chains enter a terminal state or all remaining indices become non-positive (hence termination), is an optimal policy. See Appendix~\ref{app:JMS-general} for more details on Gittins indices and the structure of such an optimal policy. Here, we only highlight that these indices can be computed in polynomial time.  

As we show in this subsection, still a refinement of the Gittins index policy above (after proper pre-processing on the Markov chains) can solve the linear optimization over the space of randomized policies $\PolicySpace$ in polynomial-time for arbitrary reward vectors $\vecreward$, where this time $\{\reward_i(s)\}$ can be arbitrarily positive or negative. In fact, we reduce the problem in polynomial-time to the special case satisfying NFL by introducing the idea of a \emph{collapsed instance}.
\begin{theorem}[\textbf{Optimal Policy for JMS with Arbitrary Rewards}]
\label{thm:JMS-optimal-reduction-informal}
Given any instance $\left\{\MC_i\right\}_{i\in[\altnum]}$ of the JMS problem, there exists a polynomial-time reduction that: (i) generates a new instance of the JMS problem satisfying NFL, called ``collapsed instance'', and (ii) by computing the Gittins indices of the collapsed instance, it returns a new set of indices $\sigma$ such that the index-based policy corresponding to $\sigma$ is optimal for the original instance of the JMS with arbitrary rewards.
\end{theorem}
We defer the proof of \Cref{thm:JMS-optimal-reduction-informal} and other technical details around our reduction to Appendix~\ref{app:JMS-general}. 
Instead, in the following section, we show how to use the resulting algorithm as a blackbox oracle to obtain a near-optimal approximate solution for \eqref{eq:opt-fair}. %\VM{Nonetheless, we emphasize that since our reduction as well as computing Gittins indices can be done in polynomial time, the resulting  oracle is also polynomial-time computable.}

==> tex/Taxation.tex <==
\newcommand{\netfunc}{N}
\newcommand{\utilagent}{U_a}
\newcommand{\utilprinc}{U_p}
\newcommand{\cdfkap}{H}
\newcommand{\start}{s}
\newcommand{\finish}{f}

\section{Fairness through Taxation}
\label{sec:taxation}

In \cref{sec:pandora} we saw how a decision maker, who wants to respect demographic parity, can adjust the optimal policy for the Pandora's Box search problem in order to find an optimal policy among all policies that satisfy the desired fairness constraint. Then in \cref{sec:general} we studied a generalized setting (model and constraints), in which again a decision maker who cares about fairness wants to implement some general ex-ante constraints into their policy for the JMS problem. Hence, the common assumption was that the decision maker itself is willing to intentionally respect such constraints. 

In this section, we take a step back, and study the situation in which there is no inherent desire for the ``searcher'' (decision maker) to satisfy some constraints. Rather, there exists a regulator (``Principal'') who - due to some societal concerns \MA{add some reference showing fairness will help in the long run} - wants to enforce such constraints to the search process of the searcher (``Agent''). Moreover, we assume that the principal lacks the ability to observe through the entire search process - due to some privacy concerns or the tremendous (labor) cost, thereby not being able to directly force the agent to satisfy the constraints and charge a huge penalty in case of violation. 

As a consequence, we consider the setting that the principal is able to charge the agent a sum depending only on the outcome of the search process, which is considered to be observable by the principal - e.g. as part of the revenue of the agent. Additionally, we assume that if the agent selects no one and decides to go with its zero reward outside option, then the principal also cannot charge agent for its zero revenue (and possibly with some costs). In particular, we consider a utility-maximizing agent who wants to search for the best alternative in the Pandora’s Box problem, but this time the principal wants to ``indirectly'' impose the demographic parity \MA{(in selection)} fairness constraint to the search process through taxing the outcome of the search $v_{i^*}$ (the revenue of the agent). \MA{send it to the last sub section} For simplicity and practical reasons, we restrict our attention to taxation policies that are deterministic from the perspective of the agent, while it can still be a priori randomized.

As for the utility function of the principal, there are three common cases that are all studied in the rest of this section. Lastly, compliant with reality and in order to make the analysis simpler, we assume that all rewards $v_i$ are non-negative. Furthermore, we also assume that at least one $\reserve_i$ from each demographic group is non-negative, as, otherwise, there is no way that agent will choose someone from that group (taxing will only hurt the value of any alternative), thereby forcing the principal to tax the other group so much that the agent will never end up selecting from that group either and always goes with the outside option of zero.  

\subsection{Social-Welfare Principal}

In the first scenario, we have a principal whose objective is to maximize the ``social welfare'', while enforcing fairness to the agent. In other words, the principal does not account for the tax payment (which is deducted from agent and given to principal) in its objective function. Accordingly, the principal's and agent's optimization problems are as follows:

\begin{align}
\label{eq:social:principal}
\tag{Principal}
\max_{\forall i\in[\altnum],v\in \mathbf{R_+}: \netfunc_i(v)\leq v }
\expect{\sum_{i\in[\altnum]} \left(\select_i^{\widetilde{\policy}}  v_i - \inspect_i^{\widetilde{\policy}}  c_i\right)},
\quad \quad ~ \textrm{s.t.} \quad  \expect{\sum_{i \in \ManSet} \select_i^{\widetilde{\policy}}} = \expect{\sum_{i \in \WomanSet } \select_i^{\widetilde{\policy}}},
\end{align}


\begin{align}
\label{eq:social:agent}
\tag{Agent}
\widetilde{\policy} \triangleq \argmax_{\policy\in\PolicySpace} \ \expect{\sum_{i\in[\altnum]} \left(\select_i^{\policy} \netfunc_i(v_i) - \inspect_i^{\policy}  c_i\right)},
\end{align}


where $\netfunc_i(v_i)\leq v_i$ is the net (after-tax) reward of alternative $i$ if its original realized reward is $v_i$. Lastly, the chosen tax function by principal for alternative $i$ would be $(I-\netfunc_i) (.) $, where $I(.)$ is the identity function.

Fortunately, the principal is able to implement the first-best solution here, i.e. get the same objective as the one it would have got by directly enforcing the adjusted optimal policy in \cref{sec:pandora}. The reason for this is that if principal selects the following  $\netfunc_i(.), \forall i\in[\altnum]$, it can get the first-best objective as in \cref{sec:pandora}. 

\begin{equation}
\label{eq:social:netvalue}
\begin{aligned}
\forall i \in [\altnum]: \quad \netfunc_i(v)\triangleq 
\begin{cases}
 v &  i \in \WomanSet~\\ 
 v-2\LagVector^* & i\in \ManSet~\\
\end{cases},
\end{aligned}
\end{equation}

where $\LagVector^*$ is the optimal Lagrange dual variable as in \cref{sec:pandora}.

To see that, its only enough to show the optimal policy chosen by the agent in \cref{eq:social:agent} will also be an optimal policy for \cref{eq:opt-FS} in \cref{sec:pandora}, which was in fact an optimal policy for \cref{eq:dual} when $\LagVector=\LagVector^*$.


\MA{complete: the lamda=0 case, and if lambda>0 the tie-breaking implementation should not change the y, and in y-preferred will decrease x by epsilon, and in x-preferred will increase x by epsilon.}


\subsection{Selfish Principal}

This situation captures the scenario when there is a principal who wants to do the search in a fair fashion, but decides to delegate this search to its agent, and in return receive a payment from the agent, and the agent can keep the rest of the profit to themselves. 

Notice that while the principal still wants to satisfy the fairness, the agent just tries to maximize its utility. In this setting, as shown in the following, the principal can extract the maximum possible expected profit to themselves, i.e. again implementing the first-best solution if principal wanted to do the search directly.


The principal's and agent's problem are as follows.



\begin{align}
\label{eq:selfish:principal}
\tag{Principal}
\max_{\forall i\in[\altnum],v\in \mathbf{R_+}: \netfunc_i(v)\leq v } \expect{\sum_{i\in[\altnum]} \select_i^{\widetilde{\policy}}  (v_i-\netfunc_i(v_i))},
\quad \quad ~ \textrm{s.t.} \quad  \expect{\sum_{i \in \ManSet} \select_i^{\widetilde{\policy}}} = \expect{\sum_{i \in \WomanSet } \select_i^{\widetilde{\policy}}},
\end{align}


\begin{align}
\label{eq:selfish:agent}
\tag{Agent}
\widetilde{\policy} \triangleq \argmax_{\policy\in\PolicySpace} \ \expect{\sum_{i\in[\altnum]} \left(\select_i^{\policy} \netfunc_i(v_i) - \inspect_i^{\policy}  c_i\right)},
\end{align}


Let us define $\utilprinc$ and $\utilagent$ as the final expected utility of the principal and agent, respectively. Now notice that $\utilprinc+\utilagent=\expect{\sum_{i\in[\altnum]} \left(\select_i^{\widetilde{\policy}}  v_i - \inspect_i^{\widetilde{\policy}}  c_i\right)}$, and also from the constraint we know $\widetilde{\policy}$ satisfies the fairness constraint. Therefore, we can deduce that $\utilprinc+\utilagent \leq \OptFairSelect$, defined in \cref{eq:opt-FS}.

Now consider the following net-reward function:

\begin{equation}
\label{eq:selfish:netvalue}
\begin{aligned}
\forall i \in [\altnum]: \quad \netfunc_i(v)\triangleq (v-\reserve_i)^+,
\end{aligned}
\end{equation}

where $\reserve_i$ is defined as in \cref{eq:base:reserve}.

As a consequence of defining $\netfunc_i(.)$ in this way, the taxed reservation values from the perspective of agent's search problem, or $\widetilde{\reserve^t_i}$ - defined in the same manner as in \cref{eq:base:reserve} when $v_i$ is replaced by $\netfunc_i(v_i)$ - will become equal to zero for the alternatives with non-negative cost, and for the negative cost alternatives $\widetilde{\reserve^t_i}$ will remain $\infty$. Now we claim that the principal can simply ask the agent to run the adjusted optimal policy derived in \cref{sec:pandora}. The reason for this is that the adjusted optimal policy in \cref{sec:pandora} is also an optimal policy for agent in this taxed version of the problem. More specifically, for the negative cost alternatives, its again always weakly better to inspect them at the beginning. After doing so, notice that, in the taxed problem, as long as a policy immediately selects an alternative after its inspection whose realized $\netfunc_i(v_i)$ is strictly greater than $\widetilde{\reserve^t_i}=0$, it will be an optimal policy for the agent in the taxed problem. Lastly, notice that the adjusted optimal policy in \cref{sec:pandora} respects this property, because:

$\netfunc_i(v_i) > \widetilde{\reserve^t_i}=0 \leftrightarrow v_i>\reserve_i \leftrightarrow \widetilde{v_i}=v_i \pm \LagVector > \reserve_i \pm \LagVector = \widetilde{\reserve_i}$,

which means that for some inspected alternative if $\netfunc_i(v_i) > \widetilde{\reserve^t_i}=0$, then $\widetilde{v_i} > \widetilde{\reserve_i}$, and finally by non-exposed property of any optimal policy for the adjusted problem, we get that the adjusted optimal policy will also select this alternative.

Finally, notice that we now have the following equations:

$\utilprinc+\utilagent = \OptFairSelect$,

$\utilagent = \sum_{\forall i \in [\altnum]} (-c_i)^+$,

where the first one is due to the fact that the adjusted optimal policy of \cref{sec:pandora} is implemented, and the second one is because all $\widetilde{\Kap^t_i}=0$ \MA{more explanation maybe?}. Finally, notice that the amount $\sum_{\forall i \in [\altnum]} (-c_i)^+$ is, indeed, a minimum guaranteed utility for the agent, as it can only inspect negative cost alternatives and then go with the outside option no matter how the principal choose its tax functions. With all this in mind, we get that $\utilprinc$ has indeed reached its maximum possible and we have found the optimal taxation policy \MA{principal is forcing the tie-break}.



\MA{fix the inconsistency that tilde here is for sec 2, and tilde+t is for tax, but later just tilde is for tax.}





\subsection{Selfless Principal}

In this last scenario, we are dealing with a principal, whose only objective is to induce the fairness to the agent's search outcome and does not personally benefit from the search itself. In other words, this case captures the situation when a regulator (principal) wants to enforce fairness with the minimum possible loss to the utility of the firm (agent) compared to the optimal unfair policy that the firm would have otherwise implemented.

For the purpose of clarity, for now suppose that the principal in addition to choosing the net function for the agent can also provide the agent a tie-breaking rule which agent will follow in case some ties occur in its search algorithm.

The problem formulation would become as follows:

\MA{need to make all 3 problem formulations to include ex-ante random net functions!}

\begin{align}
\label{eq:selfless:principal}
\tag{Principal}
\max_{(\netfunc_1,...,\netfunc_n)=\mathbf{\netfunc} \sim \mathcal{\netfunc}, \tiebreak \sim \mathcal{T}\big | \mathbf{\netfunc} }
\expect{ \expect{ \sum_{i\in[\altnum]} \left(\select_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}} \netfunc_i(v_i) - \inspect_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}}  c_i\right) \Big | ~ \mathbf{\netfunc}, \tiebreak}}
,
\quad ~ \textrm{s.t.} \quad  \expect{\sum_{i \in \ManSet} \select_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}}} = \expect{\sum_{i \in \WomanSet } \select_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}}},
\end{align}


\begin{align}
\label{eq:selfless:agent}
\tag{Agent}
\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}} \triangleq \argmax_{\policy\in\PolicySpace} \ \expect{\sum_{i\in[\altnum]} \left(\select_i^{\policy} \netfunc_i(v_i) - \inspect_i^{\policy}  c_i\right) \Bigg | ~ \mathbf{\netfunc},\tiebreak},
\end{align}

where $\mathcal{\netfunc}$ -- a distribution over tuple of deterministic net functions $(\netfunc_1(.),...,\netfunc_n(.))$, such that $\forall i\in[\altnum],v\in \mathbf{R_+}: \netfunc_i(v)\leq v$ -- and $\mathcal{T}\big | \mathbf{\netfunc}$ -- the conditional distribution over different tie-breaking rules conditioned on the net function -- are the decision variables of the principal. 

\MA{how can we write the distribution better?}

Before, going to the details of the analysis, notice that due to the assumption that from the agent's perspective the tax function is a deterministic function as well as the fact that $\forall i \in [\altnum],\ v_i$ is a discrete random variable, we can deduce that $\forall i \in [\altnum],\ \netfunc_i(v_i)$ is also a discrete random variable w.r.t. $v_i$ (conditional on $\mathbf{\netfunc}$).



Now we will start analyzing this problem. In order to get the optimal taxation, first we check whether there exists an optimal solution without any taxation, because if there is, then clearly implementing that policy will be the optimal solution for the taxed problem as well. Similar to the \cref{sec:pandora}, its enough to study the most-extreme optimal policies for agent in the no-adjustment problem, i.e. the group preferred tie-breaking rules introduced in \cref{def:tie:FS}. 

If the {\em FS slack} for the \emph{$\WomanSet$-preferred rule} is non-negative and for the \emph{$\ManSet$-preferred rule} is non-positive, then the only remaining thing for the principal to do is to just make the agent to run those two tie-breaks with appropriate probabilities, ex-ante. \MA{send the rest of the paragraph to remark} Lastly, the way that the principal will induce those tie-breaking rules is as following. Suppose, the principal wants to induce the \emph{$\WomanSet$-preferred rule}. From \cref{sec:pandora} we know that one way to do it is to add an infinitesimal positive $\epsilon$ to all alternatives in $\WomanSet$, and deduce $\epsilon$ from everyone in $\ManSet$. However, if $\exists i\in\WomanSet, v: \netfunc_i(v)=v$, then it is impossible to increase the net reward by some positive amount for that alternative and not violate the $\netfunc_i(v) \leq v$ constraint. Alternatively, another equivalent way to induce the same tie-break is to just reduce the $\netfunc_i(v), \forall i \in \ManSet$, by an infinitesimal positive $\epsilon$, and keep the alternatives from $\WomanSet$ unchanged. By doing so, we are again de-prioritizing alternatives in $\ManSet$, and, as for the ones in $\WomanSet$, they will automatically get prioritized over the outside option, simply due to the assumption that we can ask the agent to prioritize choosing someone from $\ManSet \cup \WomanSet$ versus the zero outside option, in case it is indifferent.

The remaining situation is either both of the slacks are positive or both of the are negative. Without loss of generality, suppose both of them are negative, so we call $\WomanSet$ the minority group and $\ManSet$ the majority group.

Now among the set of all optimal taxation \MA{possibly random!}, consider the one with maximal $\{\netfunc_i(.)\}_{i\in \WomanSet}$ \MA{is it clear?}. The following lemma shows us in such optimal taxation we should have $\forall i \in \WomanSet, v: \netfunc_i(v)=v$, almost surely.

\MA{we can also say there exist an optimal tax dist. that doesn't tax minority, is it better?}

\begin{lemma}
The maximal taxation, defined as above, will not tax any alternative from the minority group ($\WomanSet$) almost surly, i.e. $\forall i \in \WomanSet, v: \netfunc_i(v)=v$ w.p. 1.
\end{lemma}

\MA{check the proof to see if consistent with dist.}

\begin{proof}{\emph{Proof.}}
We prove the lemma by contradiction. Suppose with positive probability $\exists i, v_i: \netfunc_i(v_i)<v_i$. Let us define a new taxation policy as follows for any realization of the net reward functions:


\begin{equation}
\begin{aligned}
\forall i \in [\altnum],v: \quad \hat{\netfunc}_i(v)\triangleq 
\begin{cases}
 v &  i \in \WomanSet~\\ 
 \netfunc_i(v) & i\in \ManSet~\\
\end{cases},
\end{aligned}
\end{equation}


Notice that as $\forall i \in \WomanSet, \ \hat{\netfunc}_i(.)\geq \netfunc_i(.)$, we get that $\hat{\Kap_i} \geq \widetilde{\Kap_i}$, where $\hat{\Kap_i}$ corresponds to the new taxed version of the problem. Additionally, $\forall i \in \ManSet, \ \hat{\netfunc}_i(.) = \netfunc_i(.)$, we get that $\hat{\Kap_i} = \widetilde{\Kap_i}$. This will tell us two important things, (i) the expected utility of the agent has weakly increased, and (ii) the {\em FS slack} is also weakly increased. Hence, this new taxation will get at least the same utility while having a non-negative slack. Finally, as we knew that the slacks for the non-taxed version of the problem (i.e. $\forall i \in [\altnum],\ \netfunc_i(v)=v$) are negative, we deduce that there is an appropriate mixing probability that we can mix $\hat{\netfunc}_i(.)$ with the non-taxed version, and get a zero {\em FS slack} while preserving at least the same utility, if not more. Hence, we have found another feasible optimal taxation whose tax functions are not equal to the $\netfunc_i(.)$ and are weakly increased, thereby contradicting the maximality assumption for $\textbf{\netfunc}$.

\qed
\end{proof}

\MA{add the assumption that we ask the agent to tie-break in favor of the $\ManSet \cup \WomanSet$ alternatives vs zero outside option}

Now that we know there exists an optimal taxation in which the minority group is not taxed at all, we restrict our attention to only such class of taxation policies, and try to find the optimal feasible policy for principal among them.

\MA{can we assume at the beginning that costs are also non-negative? this will make the utility of the agent to be exactly equal to the E[max kappa]}


First, we state the Lagrangian dual of the principal's problem in the following:


\begin{align}
\label{eq:selfless:lagrange-dual}
\tag{Lagrange-Dual}
\min_{\LagVector} \left\{ \max_{(\netfunc_1,...,\netfunc_n)=\mathbf{\netfunc} \sim \mathcal{\netfunc}, \tiebreak \sim \mathcal{T}\big | \mathbf{\netfunc} }
\expect{ \expect{ \sum_{i\in[\altnum]} \left(\select_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}} \netfunc_i(v_i) - \inspect_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}}  c_i\right) + \LagVector \left( \sum_{i \in \WomanSet} \select_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}} - \sum_{i \in \ManSet } \select_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}} \right)  \Big | ~ \mathbf{\netfunc}, \tiebreak}} \right\},
\end{align}

\MA{let us assume that all costs are positive, as we want that y-preferred to be the unique maximizer of slack. However, we don't even need it to be the unique maximizer of slack , as any two optimal tie-break should have the same slack and thus does not matter in the saddle point. Do we need to explain it?}


First of all, notice that the dual objective is yet again a convex function w.r.t. $\LagVector$, as given any distribution over net functions and tie-breaks the Lagrangian is a linear function of $\LagVector$, and we are taking sup over all distributions. \MA{is it true that sup is convex even in infinite dim case?}

If $\LagVector^*=0$, the primal player's objective will be to just maximize the utility of the agent, which means that the principal wants to induce fairness without any loss in the objective of the agent, and this case goes back to our previous discussion that the {\em FS slack} for \emph{$\WomanSet$-preferred rule} (resp. \emph{$\ManSet$-preferred rule}) should be non-negative (resp. non-positive) so that the principal can satisfy the fairness. However, we know that both of these {\em FS slack}s are negative, which will tell us that $\LagVector^*>0$, since the {\em FS slack} term at any $\LagVector$ for any best response of the primal player would be again a sub-gradient of the Lagrange dual function at $\LagVector$. 

Notice that the tie-breaking (by definition) will not affect the utility of the agent, which is exactly the first summation in the inner expectation. As a consequence, the primal player when maximizing over the tie-breaking distributions, will always ask for the tie-breaking rule that maximizes the {\em FS slack} (we knew $\LagVector>0$), which indeed would be the \emph{$\WomanSet$-preferred rule}. \MA{again there could be other optimal tie-breaks but all should have same slack and hence does not matter in the constraint, and saddle point.}


Next, we state that in such class of principal's policies (no tax for minority group $\WomanSet$ as well as \emph{$\WomanSet$-preferred rule}) the agent will never select the zero outside option, no matter how much tax principal is taking for the majority group. This is simply because we know that: (i) all before-tax rewards are non-negative, (ii) there was an alternative in each group with non-negative before-tax reservation value $\reserve_i$, (iii) minority group are not taxed, and (iv) the agent was asked to tie-break in favor of $\WomanSet$. \MA{does it need more explanation?}


Additionally, as for the distribution over net functions of the majority group, without loss of generality, we can assume it is non-negative almost surly. This again follows from the fact that the minority group are not taxed and the agent is running $\emph{$\WomanSet$-preferred rule})$, so regardless of whether the net reward of some alternatives in majority group are zero or negative, the agent will not choose them, because there is at least one alternative in the minority group weakly better than them. Therefore, truncating the net functions to be at least zero will not affect the utility of the agent nor the {\em FS slack}, and we can further restrict our attention to the class of non-negative net functions to find the optimal policy of the principal.




We will now try to find out the set of best response distributions by the primal player (principal). As we are considering distributions over deterministic net functions, a distribution is a best response if and only if all of its mass is on some deterministic best response net functions. Hence, the set of best response distributions are all distributions over the set of all deterministic best response net functions. In the following we will characterize this set.

Consider some deterministic net functions $\mathbf{\netfunc}$, and $\tiebreak$ to be the $\emph{$\WomanSet$-preferred rule})$. Now let us define $\forall i \in [\altnum],\ \cdfkap_i$ (resp. $\cdfkap_i'$) as the cumulative (resp. probability) density function for the random variable $\Kap_i$. Notice that $\cdfkap_i'$ only consists of some Dirac delta functions. We further define $\cdfkap_\WomanSet$ and $\cdfkap_\ManSet$ (resp. $\cdfkap_\WomanSet'$ and $\cdfkap_\ManSet'$) as the cdf (resp. pdf) for the random variable of $\max_{i\in \WomanSet} \Kap_i$ and  $\max_{i\in \ManSet} \Kap_i$, respectively.

For brevity of notation, in this part, whenever we use $\widetilde{\Box}$, we mean the $\Box$ for the taxed version of the problem, with net functions as in $\mathbf{\netfunc}$. For instance, $\widetilde{\cdfkap_\ManSet}'$, is defined as the pdf of $\max_{i\in \ManSet} \widetilde{\Kap_i}$, which again only consists of some Dirac delta function too. Furthermore, since $\forall i \in \ManSet, v: \netfunc_i(v)\leq v \rightarrow \widetilde{\Kap_i} \leq \Kap_i$ and $\forall i \in \WomanSet, v: \netfunc_i(v)= v \rightarrow \widetilde{\Kap_i} = \Kap_i$ , we deduce that $\widetilde{\cdfkap_\WomanSet} = \cdfkap_\WomanSet$ and $\widetilde{\cdfkap_\ManSet} \geq \cdfkap_\ManSet$. 



Due to the fact that agent will always select an alternative, we have:

\begin{align}
\expect{\left( \sum_{i \in \WomanSet} \select_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}} - \sum_{i \in \ManSet } \select_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}} \right)  \Big | ~ \mathbf{\netfunc}, \tiebreak} = 2 ~ \expect{\sum_{i \in \WomanSet} \select_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}}  \Big | ~ \mathbf{\netfunc}, \tiebreak}-1 
& = 2 ~ \prob{\max_{i\in \WomanSet} \widetilde{\Kap_i} \geq \max_{i\in \ManSet} \widetilde{\Kap_i}} - 1 \nonumber\\
& = 2\int_0^\infty \cdfkap_\WomanSet'(u) \times \widetilde{\cdfkap_\ManSet} (u) ~ du - 1
\end{align}

We can also rewrite the agent's utility function, or the expectation of first summation in the Lagrangian as:



\begin{align}
\expect{ \sum_{i\in[\altnum]} \left(\select_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}} \netfunc_i(v_i) - \inspect_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}}  c_i\right)  \Big | ~ \mathbf{\netfunc}, \tiebreak} = \int_0^\infty 1 - \cdfkap_\WomanSet(u) \times \widetilde{\cdfkap_\ManSet} (u) ~ du
\end{align}


Accordingly, we can write the Primal's best response problem among deterministic net functions $\mathbf{\netfunc}$ as:


\begin{align}
\label{eq:selfless:primal-bestresponse}
\max_{(\netfunc_1,...,\netfunc_n)=\mathbf{\netfunc} }
\expect{ \sum_{i\in[\altnum]} \left(\select_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}} \netfunc_i(v_i) - \inspect_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}}  c_i\right) + \LagVector \left( \sum_{i \in \WomanSet} \select_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}} - \sum_{i \in \ManSet } \select_i^{\widetilde{\policy_{\mathbf{\netfunc},\tiebreak}}} \right)  \Big | ~ \mathbf{\netfunc}, \tiebreak} \\
\tag{Primal's best response}
= \int_0^\infty 1 - \left( \cdfkap_\WomanSet(u) - 2\LagVector \cdfkap_\WomanSet'(u) \right) \times \widetilde{\cdfkap_\ManSet} (u) ~ du - \LagVector
\end{align}




Consequently, instead of finding optimal $\mathbf{\netfunc}$ we can find the optimal $\widetilde{\cdfkap_\ManSet} (u)$ that maximizes the above expression, and satisfies cdf properites of a FOSD discrete random variable $\max_{i\in \ManSet} \widetilde{\Kap_i}$, i.e. (i) $1 \geq \widetilde{\cdfkap_\ManSet} (u) \geq \cdfkap_\ManSet$, (ii) $\widetilde{\cdfkap_\ManSet} (u)$ is non-decreasing, piece-wise constant with finite jumps, and right continuous. 

\begin{remark}
Notice that not any function $\widetilde{\cdfkap_\ManSet} (u)$ that satisfies the above conditions can be the cdf of $\max_{i\in \ManSet} \widetilde{\Kap_i}$ for some net functions (taxation). However, as you will see in the rest of this section, the ones we will drive as some optimal solutions are indeed among the achievable ones.
\end{remark}

In the following, we state our main theorem for this section, that characterizes the optimal taxation policy that should be used by the principal.

\begin{theorem} {\bf Optimal Taxation}
There is a sequence of real numbers: $0\leq \start_1 < \finish_1 \leq \start_2 < \finish_2 \leq ... \leq \start_k < \finish_k$ such that an optimal distribution over net functions would be a mixing over the following two net functions, with an appropriate probability that makes the {\em FS slack} zero:


\begin{enumerate}
    \item  Minimal optimal tax: 
    \begin{align}
        \forall i \in \WomanSet: \quad \netfunc_i(v)\triangleq v, \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \ \nonumber\\
        \forall i \in \ManSet, \nexists ~ 1\leq j: \start_j\leq \reserve_i < \finish_j : \quad \netfunc_i(v)\triangleq 
        \begin{cases}
         \start_l & \exists ~ 1\leq l: \start_l\leq v < \finish_l \leq \reserve_i~\\ 
         v & o.w.~\\
        \end{cases} \quad\quad\quad\quad, \nonumber\\
        \forall i \in \ManSet, \exists ~ 1\leq j: \start_j\leq \reserve_i < \finish_j: \quad \netfunc_i(v)\triangleq
        \begin{cases}
         \start_l & \exists ~ 1\leq l<j: \start_l\leq v < \finish_l~\\ 
         \start_j & \start_j\leq v < \reserve_i~\\ 
         v-(\reserve_i-\start_j) & \reserve_i \leq v ~\\
         v & o.w.~\\
        \end{cases}, \nonumber
    \end{align}
    \\
    \item Maximal optimal tax:
    \begin{align}
        \forall i \in \WomanSet: \quad \netfunc_i(v)\triangleq v, \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad   \nonumber\\
        \forall i \in \ManSet, \nexists ~ 1\leq j: \start_{d_{j-1}+1}\leq \reserve_i < \finish_{d_j} : \quad \netfunc_i(v)\triangleq 
        \begin{cases}
         \start_{d_{l-1}+1} & \exists ~ 1\leq l: \start_{d_{l-1}+1}\leq v < \finish_{d_l} \leq \reserve_i~\\ 
         v & o.w.~\\
        \end{cases} \quad\quad\quad\quad, \nonumber\\
        \forall i \in \ManSet, \exists ~ 1\leq j: \start_{d_{j-1}+1}\leq \reserve_i < \finish_{d_j}: \quad \netfunc_i(v)\triangleq
        \begin{cases}
         \start_{d_{l-1}+1} & \exists ~ 1\leq l<j: \start_{d_{l-1}+1}\leq v < \finish_{d_l}~\\ 
         \start_{d_{j-1}+1} & \start_{d_{j-1}+1}\leq v < \reserve_i~\\ 
         v-(\reserve_i-\start_{d_{j-1}+1}) & \reserve_i \leq v ~\\
         v & o.w.~\\
        \end{cases}, \nonumber
    \end{align}

\end{enumerate}

where $d_0 \triangleq -1$, $s_0 \triangleq 0$, and for any $1\leq j$, $d_j$ is the $j$-th $f$ which is not equal to the next $s$.
\end{theorem}



\begin{proof}{\emph{Proof.}}
As discussed above (\cref{eq:selfless:primal-bestresponse}), given any $\LagVector$ we try to find the set of optimal $\widetilde{\cdfkap_\ManSet} (u)$ that minimizes the following, while satisfying the mentioned properties:

\begin{align}
\label{eq:selfless:obj-taxedcdf}
\tag{Opt CDF}
    \min_{\widetilde{\cdfkap_\ManSet} (.)} \int_0^\infty \left( \cdfkap_\WomanSet(u) - 2\LagVector \cdfkap_\WomanSet'(u) \right) \times \widetilde{\cdfkap_\ManSet} (u) ~ du
\end{align}

Next we will provide the derivation for the sequence $0\leq \start_1 < \finish_1 \leq \start_2 < \finish_2 \leq ... \leq \start_k < \finish_k$ mentioned in the theorem. The elements of the sequence will be built sequentially as follows, until no more $s_j$ exists:

$i \leftarrow 1$

$0\leq s_i \triangleq \inf \{ v | \cdfkap_\WomanSet(v^-)<\cdfkap_\WomanSet(v^+) \}$,

$f_i \triangleq \inf \{ v > s_i | \int_{s_i^-}^{v^-} \left( \cdfkap_\WomanSet(u) - 2\LagVector \cdfkap_\WomanSet'(u) \right) ~ du = 0 \} $

While $\cdfkap_\WomanSet(f_i^-)<1$:

$\bullet \quad s_{i+1} \triangleq \inf \{ v \geq f_i | \cdfkap_\WomanSet(v^-)<\cdfkap_\WomanSet(v^+) \}$

$\bullet \quad f_{i+1} \triangleq \inf \{ v > s_{i+1} | \int_{s_{i+1}^-}^{v^-} \left( \cdfkap_\WomanSet(u) - 2\LagVector \cdfkap_\WomanSet'(u) \right) ~ du = 0 \} $

$\bullet \quad i \leftarrow i+1$

We will now provide some claims:

\begin{claim}
Any optimal $\widetilde{\cdfkap_\ManSet} (.)$ must be a constant function over interval $[s_i,f_i)$, for any $i$.
\end{claim}
\begin{proof}{\emph{Proof.}}
The proof simply follows from the fact that for any $v \in (s_i,f_i)$ we have $\int_{s_{i}^-}^{v^-} \left( \cdfkap_\WomanSet(u) - 2\LagVector \cdfkap_\WomanSet'(u) \right) ~ du < 0$. As a consequence, if there is a jump in $\widetilde{\cdfkap_\ManSet} (.)$ at $v$, then by increasing $\widetilde{\cdfkap_\ManSet} (.)$ in a uniform fashion on the interval $[s_i,v)$ until the jump vanishes, we are able to strictly decrease \cref{eq:selfless:obj-taxedcdf}, contradicting with optimality of $\widetilde{\cdfkap_\ManSet} (.)$. This fact in addition to the right continuity of $\widetilde{\cdfkap_\ManSet} (.)$ will conclude the proof of this claim.
\qed
\end{proof}


\begin{claim}
If we define $s_{k+1}=\infty$, then $\forall 1 \leq i \leq k,~ s.t. ~ f_i<s_{i+1}$, we must have $\widetilde{\cdfkap_\ManSet} (u) = \cdfkap_\ManSet (u)$, $\forall u \in [f_i,s_{i+1})$.  
\end{claim}
\begin{proof}{\emph{Proof.}}
We prove this claim again by contradiction. Suppose $\exists i, v, f_i\leq v < s_{i+1}$, $\widetilde{\cdfkap_\ManSet} (v) > \cdfkap_\ManSet (v)$. By the fact that both of $\widetilde{\cdfkap_\ManSet} (.)$ and $\cdfkap_\ManSet (.)$ are cdf of a discrete random variable and are right continuous, we can deduce that $\exists 0<\epsilon<s_{i+1}-v$ such that $\widetilde{\cdfkap_\ManSet} (v+\epsilon) = \widetilde{\cdfkap_\ManSet} (v) > \cdfkap_\ManSet (v) = \cdfkap_\ManSet (v+\epsilon)$. Moreover, from the fact that $f_i<v+\epsilon<s_{i+1}$ as well as the way we defined our sequence we can deduce that $\forall a<v+\epsilon$, we have $\int_{a^-}^{v+\epsilon^-} \left( \cdfkap_\WomanSet(u) - 2\LagVector \cdfkap_\WomanSet'(u) \right) ~ du > 0$. This means that if we consider the last jump in $\widetilde{\cdfkap_\ManSet} (.)$ before $v+\epsilon$, call it $a ~ (\leq v)$, and reduce $\widetilde{\cdfkap_\ManSet} (.)$ in a uniform fashion on the interval $[a,v+\epsilon)$, until either the jump at $a$ vanishes or $\widetilde{\cdfkap_\ManSet} (v)$ becomes equal to $\cdfkap_\ManSet (v)$, then we are able to again strictly decrease \cref{eq:selfless:obj-taxedcdf}, contradicting with optimality of $\widetilde{\cdfkap_\ManSet} (.)$.
\qed
\end{proof}


With all this in mind, the only degrees of freedom left for the set of optimal $\widetilde{\cdfkap_\ManSet} (.)$, are its value in $[0,s_1)$, as well as the level of those constant functions. Furthermore, notice that as long as we respect $\widetilde{\cdfkap_\ManSet} (.)\geq \cdfkap_\ManSet (.)$ and monotone increasing property (our feasibility constraints on the form of the $\widetilde{\cdfkap_\ManSet} (.)$), the value of \cref{eq:selfless:obj-taxedcdf} would be the same no matter how we determine those degrees of freedom. This is simply due to the fact that $\forall u \in [0,s_1), \left( \cdfkap_\WomanSet(u) - 2\LagVector \cdfkap_\WomanSet'(u) \right) =0$, and $\forall i, \int_{s_{i}^-}^{f_{i}^-} \left( \cdfkap_\WomanSet(u) - 2\LagVector \cdfkap_\WomanSet'(u) \right) ~ du = 0$.

Additionally, notice that this set of best response solutions adhere a maximum (resp. minimum) CDF, corresponding to maximum (resp. minimum) taxation for alternatives in group $\ManSet$. Hence, these two taxation policies will indeed get the maximum (resp. minimum) {\em FS slack} among all taxation policies that are best response to $\LagVector$. 

In the end, either, if we find the $\LagVector^*$ (the optimal dual solution), or we find two $\LagVector^+,\LagVector^-$ with $|\LagVector^+ - \LagVector^-|<\epsilon$ for which the {\em FS slack} is non-negative and non-positive, respectively, ...

\qed
\end{proof}



















\MA{below will go under remark on how to implement y-preferred rule.}




Additionally, with the same procedure as above, given any taxation, the principal can implement group preferred tie-breaking rules by just reducing the $\netfunc_i(.)$ for all alternatives in the opposite group with infinitesimal $\epsilon>0$ and loosing at most $\epsilon$ in the objective function. \MA{is the explanation enough?}

Hence, first we can further restrict our attention to only those policies for which a tie in deciding between $\WomanSet$ and $\ManSet$ never happens, and loose at most an additive $\epsilon>0$. Next, we expand our attention, by now considering the previous set of tax polices (that still do not tax the minority) \MA{naming the such sets of policies are helpful I guess?} and now we imagine that the agent itself will always tie-break in favor of the minority group $\WomanSet$. Now if we find an optimal tax policy within this assumption, then again by loosing at most another $\epsilon>0$, we can take the burden of tie-breaking between $\WomanSet$ and $\ManSet$ off the shoulders of the agent and implicitly incorporating it in the perturbed taxation similar to the above. Therefore, the final solution will have an additive error of at most $2\epsilon$.


To sum up the above, from now on, we know that: (i) the principal will not tax $\WomanSet$, and (ii) the agent prioritize $\WomanSet$ over the outside option as well as $\ManSet$. 

==> tex/app_copy2_Exact_Caratheodory.tex <==


\newcommand{\epsilonVector}{\overrightarrow{\varepsilon}}


\revcolorm{
\section{Technical Details of \Cref{sec:caratheodory}: Exact Optimal Policy for Pandora's box with Multiple Ex-ante Affine Constraints}
\label{app:mutiple-affine}

\RN{these two subsections and the pre-amble should be majorly revised; they are quite bad}

% In this section, we first provide an example illustrating the importance on the tie-breaking rules that should be used to satisfy the fairness constraint(s), especially when we have $\numaffine>1$ constraints to satisfy. In particular, restricting our attention only to perturbations of the form $\{+\epsilon , -\epsilon\}^m$ is not enough. 

% Realizing the shortcoming of this approach, we next provide a polynomial-time algorithm that extends our exact optimal solutions for the single affine constraint to the setting with $\numaffine>1$ number of such constraints. 

% Before showing that, in \Cref{subsection: Exact Carathéodory problem}, we first state an abstraction from this problem to a geometric problem which we call ``Exact Carathéodory problem" and show how we can solve this problem. Then, in \Cref{subsection: reduction of equality constrained to Caratheodory} we show how our original problem that only have equality constraints can be reduced to this Exact Carathéodory problem. Lastly, in \Cref{subsec: reduction of inequality to equality}, we show how we can reduce a general problem with multiple affine inequality and equality constraints to a one with only equality constraints.



In this section, we begin by presenting an example, in \Cref{app:extreme-failure-multiple-affine} that highlights the significance of the tie-breaking rules necessary to fulfill fairness constraints, particularly when there are $\numaffine > 1$ constraints to consider. Notably, focusing solely on perturbations of the form $\{+\epsilon, -\epsilon\}^m$ proves insufficient.

Recognizing this limitation, we subsequently introduce a polynomial-time algorithm that generalizes our exact optimal solutions for a single affine constraint to cases with $\numaffine > 1$ constraints. Before presenting this algorithm, in \Cref{subsection: Exact Carathéodory problem}, we formalize an abstraction of the original problem into a geometric problem, which we term the "Exact Carathéodory problem," and demonstrate our solution method. Then, in \Cref{subsection: reduction of equality constrained to Caratheodory}, we illustrate how our initial problem—comprising only equality constraints—can be transformed into this Exact Carathéodory problem. Finally, in \Cref{subsec: reduction of inequality to equality}, we explain how a general problem with multiple affine inequality and equality constraints can be reduced to one involving only equality constraints.






\subsection{$2^\numaffine$ tie-breaks derived by $\{+\epsilon , -\epsilon\}^m$ perturbations is insufficient for $\numaffine>1$!}
\label{app:extreme-failure-multiple-affine}

In this section we provide an illustrative example showing why a naive generalization of our approach for the single constraint setting cannot always provide us with a subset of policies that enables achieving a zero slack in all of the constraints, at the same time, by randomizing over these policies.

More specifically, when we had a single affine constraint ($\numaffine=1$), we saw in \Cref{sec:randomized-tie} that the two tie-break orders induced by the perturbed optimal dual variables $\LagVector^*-\varepsilon$ and $\LagVector^*+\varepsilon$ will indeed result in the two most extreme slack (highest and lowest) in the constraint among all possible tie-breaking orders. As a consequence, one of them should be non-negative and the other one should be non-positive, enabling a zero slack by randomizing over them. Given this simple structure, it is quite reasonable to consider generalizing this idea to the settings with multiple constraints ($\numaffine>1)$. Mathematically speaking, adding an infinitesimal vector $\epsilonVector \in \{-\varepsilon, +\varepsilon\}^\numaffine$ to the optimal dual variable $\LagVector^*\in \reals^\numaffine$. However, this approach may not always work due to the following two reasons. The first reason, which is easy to expect, is the computational complexity of this approach. In particular, the running time would be exponential w.r.t. $\numaffine$, making it impractical for real world implimentations, as $\numaffine$ becomes large. Notwithstanding, this approach seems appropriate for small $\numaffine$. This brings us to the second, more subtle reason that we explain in the rest of this section. 

Denote by $P$ the set of all subgradients of the dual function $\DualLagrangeConst (\LagVector)$ at $\LagVector=\LagVector^*$. Notice that $P$ constructs a polytope in $\reals^\numaffine$ that may consist of exponential number of vertices w.r.t. $n$ (the number of boxes). With this representation, the problem translates to finding a subset of vertices of $P$ - each of which corresponds to the vector of constraints' slacks $(\slack)$ associated with some tie-breaking rule - such that their convex combination can cover $\origin$. Now, when $\numaffine>1$, we no longer can guarantee that if we find the $2^\numaffine$ points in $P$ corresponding to the slack of tie-breaking rules derived from the $\epsilonVector \in \{-\varepsilon, +\varepsilon\}^\numaffine$ perturbations on $\LagVector^*$, we would be able to cover $\origin$ with them. The following plot clarifies the source of this phenomenon through a simple, high-level example. Suppose $\numaffine=2$ and there are only 4 possible tie-breaking rules, whose slacks are represented by the blue points in the plot. As can be seen from the plot, one can cover $\origin$ by randomizing over all 4 of these points. Nevertheless, those $2^2$ directions derived from aforementioned perturbations will only result in two distinct tie-breakings, the two farthest points from the $\origin$, with which we cannot cover $\origin$.


\begin{center}
\begin{tikzpicture}
    \begin{axis}[
        axis lines = middle,
        xlabel = {$x$},
        ylabel = {$y$},
        xmin=-5, xmax=5,
        ymin=-5, ymax=5,
        grid=both,
        % legend style={at={(1.1,1.1)},anchor=north east, scale=0.1}
    ]
    
    % Draw points
    \addplot[
        only marks,
        mark=*,
        color=blue,
        ] coordinates {
        (0.5,1) (-1,-1.5) (4,2) (-3,-2)
    };

    % Draw 2 special points
    \addplot[
        only marks,
        mark= square*,
        color=purple,
        ] coordinates {
        (4,2) (-3,-2)
    };
    
    % Connect the outer points
    \addplot[
        color=green,
        thick
        ] coordinates {
        (-3,-2) (0.5,1) (4,2) (-1,-1.5) (-3,-2) 
    };
    % Connect the outer points
    \addplot[
        color=red,
        thick
        ] coordinates {
        (4,2) (-3,-2) 
    };
    
    % Draw bisectors
    \addplot[
        domain=-4:4, 
        samples=100, 
        color=black, 
        dashed
    ] {x}; % y = x (1st diagonal)
    
    \addplot[
        domain=-4:4, 
        samples=100, 
        color=black, 
        dashed
    ] {-x}; % y = -x (2nd diagonal)
    
    % \addplot[
    %     domain=-4:4, 
    %     samples=100, 
    %     color=black, 
    %     dashed
    % ] {0}; % Horizontal bisector (y = 0)
    
    % \addplot[
    %     domain=-3:3, 
    %     samples=100, 
    %     color=black, 
    %     dashed
    % ] (0,x); % Vertical bisector (x = 0)

    % \legend{Points, Outer Points Connection, $y=x$, $y=-x$, Horizontal Bisector, Vertical Bisector}

    \end{axis}
\end{tikzpicture}
\end{center}


In the following, we provide a stylized class of numerical examples that rigorously demonstrates this fact.

In these class of examples we have only 3 boxes, boxes 1 and 2 belong to $\ManSet$ and box 3 belongs to $\WomanSet$. Each box has a binary random valuation as follows:

\begin{align}
    v_1 \sim F_1 \triangleq 
    \begin{cases}
        H_1 \quad w.p. \ p_1 =1,\\
        L_1 \quad w.p. \ 1-p_1 =0,
    \end{cases}
    v_2 \sim F_2 \triangleq 
    \begin{cases}
        H_2 \quad w.p. \ p_2,\\
        L_2 \quad w.p. \ 1-p_2,
    \end{cases}
    v_3 \sim F_3 \triangleq 
    \begin{cases}
        H_3 \quad w.p. \ p_3,\\
        L_3 \quad w.p. \ 1-p_3,
    \end{cases}
\end{align}

For brevity of exposition, we abstract away from setting the exact numerical values of $H_i,\ L_i,\ c_i\ \textrm{(cost)},\ \reserve_i\ \textrm{(indices as defined in \Cref{eq:base:reserve})}, \forall i\in[3],$ and only require them to satisfy the following comparative relation. Nevertheless, we note that this relation can be easily satisfied by a large class of numerical values.
\begin{align}
    \min(H_1,H_2,H_3) > \reserve_1 = \reserve_2 = \reserve_3 > L_3 > \max (L_1,L_2). 
\end{align}
This relation is essentially ensuring that an optimal policy would stop if and only if 1) it sees a high value and select it, or 2) it has already inspected all 3 boxes (all with low values), and then selects the third box. For simplicity, suppose that $p_1=1$.

As for the constraints, suppose the decision maker wants to satisfy (normalized version of) both equal opportunity and equal outcome at the same time. Mathematically speaking:
\begin{equation}
\label{eq:normalized parity}
\tag{Normalized Parity}
        \expect{\select_1^{\policy} + \select_2^{\policy} } = 2 * \expect{\select_3^{\policy}}~~ \textrm{AND}~~~ \expect{\inspect_1^{\policy} + \inspect_2^{\policy} } = 2 * \expect{\inspect_3^{\policy}}.
\end{equation}

With this setting in mind, note that because all three indices are equal, we can have arbitrary permutations on them. In fact, again in this example the loss due to fairness is designed to be 0, meaning that $\LagVector=\origin$, to focus the attention on the importance exactly which tie-breaking to choose. It's easy to simply shift things around, to make some adjustments necessary ($\LagVector \neq \origin$). To this end, we show that it is indeed not possible to achieve a $\origin$ slack by only considering the $2^2$ (potentially non-distinct) tie-breakings derived from symmetric perturbations. However, by adding another tie-breaking (corresponding to some non-bisect direction) to the consideration set, we can cover $\origin$, and thus no price of fairness.

The following 6 orders capture all possible ways to tie-break. Its not hard to compute the resulting slack in \ref{eq:normalized parity} for inspection (selection), denoted by $\slack_I$ ($\slack_S$).

\begin{enumerate}
    \item $1 \rightarrow 2 \rightarrow 3$:
    $\slack_I=1, \slack_S=1$

    \item $2 \rightarrow 1 \rightarrow 3$:
    $\slack_I=2-p_2=1.25, \slack_S=1$
    
    \item $3 \rightarrow 1 \rightarrow 2$: 
    $\slack_I=-(1+p_3)=-1.85, \slack_S=1-3p_3=-1.55$
    
    \item $3 \rightarrow 2 \rightarrow 1$:
    $\slack_I=p_2p_3-p_2-2p_3=-1.8125, \slack_S=1-3p_3=-1.55$
    
    \item $1 \rightarrow 3 \rightarrow 2$:
    $\slack_I=1, \slack_S=1$
    
    \item $2 \rightarrow 3 \rightarrow 1$:
    $\slack_I=p_2p_3+p_2-p_3=0.5375, \slack_S=1-3p_3+3p_2p_3=0.3625$
\end{enumerate}

Now it turns out that if we have
$$\frac{2}{p_3}-\frac{1}{p_2}>1,$$
then two of the four tie-breaking rules derived by $\{-\varepsilon, +\varepsilon\}^2$ are actually redundant, and we will only discover those in item 2 and 3. As explained before and illustrate in the following plot, under the configuration of $p_2$ and $p_3$ shown in \Cref{fig: probability region}, we can observe that item 2 and 3 are not enough to cover $\origin$, but once we also include the item 1, then we will be able to cover $\origin$. \Cref{fig:6 point example_a} shows the configuration of all 6 points, setting $p_2=0.75, p_3=0.85$. In \Cref{fig:6 point example_b}, you can see similar results for $p_2=0.7, p_3=0.8$


\begin{figure}[htb]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/probability_region.pdf}
        \caption{x-axis and y-axis represents $p_3$ and $p_2$ respectively.}
        \label{fig: probability region}
    \end{subfigure}
    \hfill 
    \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \label{fig:6 point example}
        \begin{tikzpicture}[scale=1]
            \begin{axis}[
                axis lines = middle,
                xlabel = {$\slack_I$},
                ylabel = {$\slack_S$},
                xmin=-2, xmax=2,
                ymin=-2, ymax=2,
                grid=both,
                % legend style={at={(1.1,1.1)},anchor=north east}
            ]
            % Plot the points
            \addplot[
                only marks,
                mark=*,
                color=blue,
                ] coordinates {
                (1, 1) (1.25, 1) (0.5375, 0.3625) (-1.8125, -1.55) (-1.85, -1.55) (1, 1) 
            };
            % highlight the 2 points
            \addplot[
                only marks,
                mark= square*,
                color=purple,
                ] coordinates {
                (1.25, 1) (-1.85, -1.55) 
            };
            % Connect the points in the given sequence
            \addplot[
                color=green,
                thick
                ] coordinates {
                (1, 1) (1.25, 1) (0.5375, 0.3625) (-1.8125, -1.55) (-1.85, -1.55) (1, 1) 
            };
            % Connect the points in the given sequence
            \addplot[
                color=red,
                thick
                ] coordinates {
                (-1.85, -1.55) (1.25, 1)
            };
            % \legend{Points, Path Connecting Points}
            \end{axis}
        \end{tikzpicture}
        \caption{Configuration of the slacks for all 6 orders, under $p_2=0.75, p_3=0.85$. The top right and bottom left belong to the two distinct tie-breaks achievable by $\{-\varepsilon, +\varepsilon\}^2$. The fact that red line does not pass through origin shows the insufficiency of this approach.}
    \end{subfigure}%
    \caption{plots}
\end{figure}


% \begin{figure}[htb]
% \label{fig:6 point example}
%     \centering
%     % First TikZ Plot
%     \begin{subfigure}{1\textwidth}
%     \label{fig:6 point example_a}
%         \centering
%         \begin{tikzpicture}
%             \begin{axis}[
%                 axis lines = middle,
%                 xlabel = {$\slack_I$},
%                 ylabel = {$\slack_S$},
%                 xmin=-2, xmax=2,
%                 ymin=-2, ymax=2,
%                 grid=both,
%                 % legend style={at={(1.1,1.1)},anchor=north east}
%             ]
            
%             % Plot the points
%             \addplot[
%                 only marks,
%                 mark=*,
%                 color=blue,
%                 ] coordinates {
%                 (1, 1) (1.25, 1) (0.5375, 0.3625) (-1.8125, -1.55) (-1.85, -1.55) (1, 1) 
%             };
            
%             % Connect the points in the given sequence
%             \addplot[
%                 color=green,
%                 thick
%                 ] coordinates {
%                 (1, 1) (1.25, 1) (0.5375, 0.3625) (-1.8125, -1.55) (-1.85, -1.55) (1, 1) 
%             };
%             % Connect the points in the given sequence
%             \addplot[
%                 color=red,
%                 thick
%                 ] coordinates {
%                 (-1.85, -1.55) (1.25, 1)
%             };
        
%             % \legend{Points, Path Connecting Points}
        
%             \end{axis}
%         \end{tikzpicture}
%         \caption{First Plot}
%     \end{subfigure}%
    % \hfill % Space between the subfigures
    % % Second TikZ Plot
    % \begin{subfigure}{0.45\textwidth}
    % \label{fig:6 point example_b}
    %     \centering
    %     \begin{tikzpicture}
    %         \begin{axis}[
    %             axis lines = middle,
    %             xlabel = {$\slack_I$},
    %             ylabel = {$\slack_S$},
    %             xmin=-2, xmax=2,
    %             ymin=-2, ymax=2,
    %             grid=both,
    %             % legend style={at={(1.1,1.1)},anchor=north east}
    %         ]
            
    %         % Plot the points
    %         \addplot[
    %             only marks,
    %             mark=*,
    %             color=blue,
    %             ] coordinates {
    %             (1, 1) (1.3, 1) (-1.8, -1.4) (-1.74, -1.4) (1, 1) (0.46, 0.28)
    %         };
            
    %         % Connect the points in the given sequence
    %         \addplot[
    %             color=green,
    %             thick
    %             ] coordinates {
    %             (1, 1) (1.3, 1) (0.46, 0.28) (-1.74, -1.4) (-1.8, -1.4)  (1, 1)
    %         };
    %         % Connect the points in the given sequence
    %         \addplot[
    %             color=red,
    %             thick
    %             ] coordinates {
    %             (-1.8, -1.4) (1.3, 1)
    %         };
        
    %         % \legend{Points, Path Connecting Points}
        
    %         \end{axis}
    %     \end{tikzpicture}
    %     \caption{Second Plot}
    % \end{subfigure}
    
%     \caption{Configuration of the slacks for all 6 orders. The top right  and bottom left belong to the two distinct tie-breaks achievable by $\{-\varepsilon, +\varepsilon\}^2$. The fact that red line does not pass through origin shows the insufficiency of this approach. a) $p_2=0.75, p_3=0.85$, b) $p_2=0.7, p_3=0.8$.}
% \end{figure}



XXX











\subsection{Exact Carathéodory problem}
\label{subsection: Exact Carathéodory problem}

First, we introduce the following definition of an Oracle, that essentially can output a solution of a linear optimization over a given polytope $P \in \reals^\numaffine$.

% %%%%%%%%%%%%%%%%%%%%%%% Oracle
\begin{definition}[Oracle($\mathfrak{h};P$)]
\label{def: Oracle_caratheodory}
    Given a polytope $P \in \reals^\numaffine$, this oracle gets as input a sequence of directions (vectors $h\in \reals^\numaffine$) $\mathfrak{h}=(h_1, h_2, ..., h_k)$, with an arbitrary $k\in \naturals$, and outputs a point $v\in \reals^\numaffine$ such that $v$ satisfies all of the following conditions:
    \begin{itemize}
        \item $A_1 := \argmax_{u'\in P} h_1.u'$
        \item $A_2 := \argmax_{u'\in A_1} h_2.u'$
        \item ... 
        \item $A_k := \argmax_{u'\in A_{k-1}} h_k.u'$
        \item $v \in A_k$.
    \end{itemize}
    If $\mathfrak{h}=(\ )$ is an empty tuple, we let $A_0:=P$, and $v$ can be any point in $A_0$. 
\end{definition}
\begin{remark}[Oracle Equivalency]
\label{remark: Oracle Equivalency}
    For any point $v$ given by the oracle defined in \Cref{def: Oracle_caratheodory} corresponding to an arbitrary sequence of directions $\mathfrak{h}=(h_1, h_2, ..., h_k)$, there exists an infinitesimal $\Bar{\varepsilon}>0$, such that for any $ 0 < \varepsilon \leq \Bar{\varepsilon}$ we have:
    \begin{align}
    \label{eq: equivalent perturbed maximizer}
        v=\argmax_{u'\in P} \Tilde{h}_{\varepsilon}.u',
    \end{align}
    where $\Tilde{h}_{\varepsilon}=\sum_{i \in [k]} h_i * \varepsilon^{(i-1)}$. Conversely, if a point $v$ satisfies \cref{eq: equivalent perturbed maximizer} for any $0 < \varepsilon \leq \Bar{\varepsilon}$, for some $\Bar{\varepsilon}>0$, then it should be the case that $v \in A_k$. This means that its equivalent to have access to an Oracle that gets as input only a single $\Tilde{h}_{\varepsilon}$. We refer to such an Oracle as a ``single-Oracle".
\end{remark}

With these, we now state the abstract problem we would like to solve:

\smallskip
\begin{displayquote}
\label{problem: exact caratheodory}
{\em
{\textbf{Problem Statement (Exact Carathéodory):}} Given an Oracle($\mathfrak{h};P$) for a polytope $P \in \reals^\numaffine$ that includes the origin $\origin \in \reals^\numaffine$ (as defined in \Cref{def: Oracle_caratheodory}), how to find, in polynomial time, a polynomial-size subset $\vertices_T$ of points in $P$, such that $\origin \in \textrm{Conv}\{\vertices_T\}$?}
\end{displayquote}

\smallskip


Let us first review some concepts and notations that we will use throughout this section.

\begin{definition}
    Let $P$ be a polytope in $\reals^\numaffine$ and $\vertices$ be a subset of its points. Denote by $\cone_{\vertices}$ the ``reverted'' cone of $\vertices$ (i.e., $\textrm{Cone}\{-\vertices\}$) and let $\dualcone_{\vertices}$ be the dual cone of $\cone_{\vertices}$, i.e., the set of all points in $\reals^\numaffine$ that have a non-negative inner product with all points in $\cone_{\vertices}$.
    % Lastly, let $\argmaxCone_{\vertices}$ be the set of all points $u$ in $P$ for which there exists a direction $d \neq \origin$ in $\dualcone_{\vertices}$ such that $u \in \argmax_{u'\in P} d.u'$.
\end{definition} 


\begin{lemma}
\label{lemma:covering}
    Suppose $\origin \in P$. For any subset of points $\vertices \subseteq P$, define $\argmaxCone_{\vertices}$ to be the set of all points $u$ in $P$ for which there exists a direction $d \neq \origin$ in $\dualcone_{\vertices}$ such that $u \in \argmax_{u'\in P} d.u'$. Then it holds:
    $$\origin \in \textrm{Conv}\{\vertices, \argmaxCone \},$$
    where $\textrm{Conv}\{A,B\} \in \reals^\numaffine$ is the convex combination of all points in $A\cup B$.
\end{lemma}

For simplicity of the notation we will drop the subscript ${\vertices}$ from the above notations, in the rest of this section. Given these notations, we now show that the following lemma holds.

\begin{proof}{\emph{Proof.}}
    Suppose $\origin \notin \textrm{Conv}\{\vertices\}$, as otherwise we are clearly done. This implies that $\cone \cap \textrm{Conv}\{\vertices\} = \phi$. With this in mind, its not hard to see that:
    \begin{align}
    \label{eq:covering_equivalency}
        \origin \in \textrm{Conv}\{\vertices, \argmaxCone \} \iff \cone \cap \textrm{Conv}\{\argmaxCone\} \neq \phi.
    \end{align}
    Additionally, we can assume that both $\vertices$ and $\argmaxCone$ are non-empty, as otherwise we have:
    \begin{itemize}
        \item if $\vertices=\phi$: then $\cone=\{\origin\} \rightarrow \dualcone=\reals^\numaffine \rightarrow \argmaxCone=P \rightarrow \origin \in P = \textrm{Conv}\{\argmaxCone\}$, and we are done.
        \item if $\argmaxCone=\phi$: then it means there was no non-zero direction in $\dualcone$, so $\dualcone = \{\origin\} \rightarrow \cone = \reals^\numaffine \rightarrow \origin \in \textrm{Conv}\{-\vertices\} \rightarrow \origin \in \textrm{Conv}\{\vertices\}$, and we are done.
    \end{itemize}
    Now, we prove RHS of \Cref{eq:covering_equivalency} by contradiction. Suppose $\cone \cap \textrm{Conv}\{\argmaxCone\} = \phi$, then there exists a strict separating hyperplane $H$ that separates $\cone$ and $\textrm{Conv}\{\argmaxCone\}$, as both of them are non-empty closed convex sets and $\textrm{Conv}\{\argmaxCone\}$ is compact. Without loss of generality we can assume that $H$ passes through $\origin$ (the only vertex of $\cone$). Let $h$ be the normal vector of $H$, pointing to the side of $H$ that includes $\cone$. We should have $h \in \dualcone$. Now, consider $u \in \argmax_{u'\in P} h.u'$, then we should have:
    \begin{equation}
    \left.
    \begin{aligned}
    & \bullet \quad h \in \dualcone \quad \rightarrow \quad u \in U \\
    & \bullet \quad \origin \in P \quad \rightarrow \quad u.h \geq 0.h = 0 \\
    & \bullet \quad \textrm{$U$ is on the other side of H as h} \quad \rightarrow \quad 0 > U.h
    \end{aligned}
    \quad\right\rbrace \rightarrow \bot \quad (\textrm{contradiction!})
    \end{equation}
    \qed
\end{proof}

Now that we have proved \Cref{lemma:covering}, we will provide our polynomial time algorithm, EEC (\ref{alg:Ellipsoid Exact Caratheodory}), to recover a subset $\vertices_T$ of the points in $P$ that cover $\origin$, i.e., $\origin \in \textrm{Conv}\{\vertices_T\}$ - assuming that we have access to the Oracle($\mathfrak{h};P$) (in other words, we can find a solution to $\argmax_{u'\in P} h.u'$ efficiently for any arbitrary direction $h \in \reals^\numaffine$).


% %%%%%%%%%%%%%%%%%%%%%%% Start of old algorithm
% \begin{algorithm}
% \caption{Ellipsoid Exact Caratheodory (EEC)}
% \label{alg:Ellipsoid Exact Caratheodory_old}
%     \SetKwInOut{Input}{input}
%     \SetKwInOut{Output}{output}
% \Input{Oracle solving $v=\argmax_{u'\in P} h.u'$ for any $h$.}

% At $t=0$: Let $\ellipse_0$ be the unit ball in $\reals^\numaffine$, and let $\centerEllipse_0=\origin$ be its center. Let $\vertices_0=\phi$.

% % Choose an arbitrary direction $h_0$ and find $v_0=\argmax_{u'\in P} h_0.u'$. Set $\vertices_0=\{v_0\}$, and construct $\cone_0, \dualcone_0$ based on $\vertices_0$. Lastly, have in mind $\argmaxCone_0$ based on $\dualcone_0$ (without characterizing it).
 
% \vspace{1mm}

% \While{$\ellipse_t \neq \{\origin\}$}{
% \vspace{1mm}
% Choose $h_t := \centerEllipse_t$, the center of ellipsoid $\ellipse_t$. If $\origin = \centerEllipse_t$, then choose an arbitrary direction $h_t$.

% Find $v_t=\argmax_{u'\in P} h_t.u'$ and set $\vertices_{t+1}:=\vertices_t \cup v_t$. 

% Define $H_t$ as the linear space orthogonal to $v_t$  and let $S_t$ be the half space of $H_t$ not including $v_t$. In other words, $H_t . v_t =0$ and $S_t . v_t \leq 0$.


% Let $\Tilde{H_t}$ be the hyper plane parallel to $H_t$ and passing through $\centerEllipse_t$, and $\Tilde{S_t}$ be its half space.

% Construct $\cone_{t+1} := \textrm{Cone}\{-\vertices_{t+1}\}=\textrm{Cone}\{\cone_{t}, - v_t\}$, $\dualcone_{t+1} := \textrm{DualCone}\{\cone_{t+1}\} = \dualcone_{t} \cap S_t$.


% Find $\ellipse_{t+1}$ as the ellipsoid constructed in the ``ellipsoid algorithm" containing $\ellipse_t \cap \Tilde{S_t}$.

% $t+=1$.
% }

% \vspace{2mm}

% \Output{set $\vertices_t$ of final nodes recovered.}
% \end{algorithm}
% %%%%%%%%%%%%%%%%%%%%%%% End of old algorithm




% %%%%%%%%%%%%%%%%%%%%%%% Start of new algorithm
\begin{algorithm}[htb]
\caption{Ellipsoid Exact Caratheodory (EEC)}
\label{alg:Ellipsoid Exact Caratheodory}
    \SetKwInOut{Input}{input}
    \SetKwInOut{Output}{output}
\Input{The Oracle($\mathfrak{h};P$) for a polytope $P \in \reals^\numaffine$ that includes the origin $\origin \in \reals^\numaffine$ (as defined in \Cref{def: Oracle_caratheodory}).}

Let $\ellipse_0$ be the unit ball in $\reals^\numaffine$, $\centerEllipse_0=\origin$ be its center, and $\vertices_0=\phi$. Also let $\ellipse_{-1}=\{\origin\}$.

{\color{orange} \# Let $\cone_{0} := \textrm{Cone}\{-\vertices_{0}\}=\{\origin\}$, $\dualcone_{0} := \textrm{DualCone}\{\cone_{0}\} = \reals^\numaffine$.}

Set $\mathfrak{h}, \Tilde{\mathfrak{h}}=(\ )$. {\color{blue} \# Empty tuples}

Set t=0.

% Choose an arbitrary direction $h_0$ and find $v_0=\argmax_{u'\in P} h_0.u'$. Set $\vertices_0=\{v_0\}$, and construct $\cone_0, \dualcone_0$ based on $\vertices_0$. Lastly, have in mind $\argmaxCone_0$ based on $\dualcone_0$ (without characterizing it).
 
\vspace{1mm}

%%%%% Outer loop starts
\While{$\ellipse_t \neq \{\origin\}$}{

Set $\mathfrak{h}=\Tilde{\mathfrak{h}}$ and $t=0$.

Let $\ellipse_0$ be the projected unit ball in $\reals^\numaffine$, where projection is done in all directions in $\mathfrak{h}$. {\color{blue} \# $\ellipse_0$ is the (lower dimensional) unit ball orthogonal to $\mathfrak{h}$}


%%%%% Inner loop starts
\While{$\ellipse_t \neq \{\origin\}$ and $\ellipse_t \neq \ellipse_{t-1}$}{
\vspace{1mm}
Choose $h_t := \centerEllipse_t$, the center of ellipsoid $\ellipse_t$, unless $\centerEllipse_t = \origin$, in which case choose an arbitrary non-zero direction $h_t \in \ellipse_t$.

Set $\Tilde{\mathfrak{h}}=concatenate(\mathfrak{h},h_t)$. {\color{blue} \# Note that $h_t \neq \origin$ is orthogonal to $\mathfrak{h}$}

Find $v_t= \textrm{Oracle}(\Tilde{\mathfrak{h}};P)$ and set $\vertices_{t+1}:=\vertices_t \cup v_t$.

\If{$v_t=\origin$}{
\textbf{return} $\vertices_t=\{v_t\}$. {\color{blue} \# The algorithm terminates, as the single point $v_t$ gives us $\origin$}
}

Define $H_t$ as the linear space orthogonal to $v_t$  and let $S_t$ be the half space of $H_t$ not including $v_t$. In other words, $H_t . v_t =0$ and $S_t . v_t \leq 0$.


Let $\Tilde{H_t}$ be the hyper plane parallel to $H_t$ and passing through $\centerEllipse_t$, and $\Tilde{S_t}$ be its half space.

{\color{orange} \# Construct $\cone_{t+1} := \textrm{Cone}\{-\vertices_{t+1}\}=\textrm{Cone}\{\cone_{t}, - v_t\}$, $\dualcone_{t+1} := \textrm{DualCone}\{\cone_{t+1}\} = \dualcone_{t} \cap S_t$.}


Find $\ellipse_{t+1}$ as the ellipsoid constructed in the ``ellipsoid algorithm" containing $\ellipse_t \cap \Tilde{S_t}$.

$t+=1$.
} %%%%% Inner loop finishes



} %%%%% Outer loop finishes


\vspace{2mm}

\Output{The last set $\vertices_t$ as the chosen set of points in $P$.}
\end{algorithm}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% End of new algorithm


We would like to show that: i) why EEC (\ref{alg:Ellipsoid Exact Caratheodory}) would terminate in polynomial time?, and ii) why its output can cover $\origin$?; which would then conclude the answer to our abstract problem (Exact Carathéodory) stated in \ref{problem: exact caratheodory}.

Before doing so, let us first state the following lemma and its important corollary.

\begin{lemma}
\label{lemma: center is out of halfspace}
    We always have $\centerEllipse_t \notin \textrm{interior } (S_t)$. Accordingly, $S_t \subseteq \Tilde{S_t}$.
\end{lemma}

\begin{proof}{\emph{Proof.}}
    First of all, if $\centerEllipse_t=\origin$, then we have $H_t=\Tilde{H_t}$ and $S_t=\Tilde{S_t}$. Else, note that, in algorithm EEC (\ref{alg:Ellipsoid Exact Caratheodory}), we set the miximization direction $h_t$ equal to $\centerEllipse_t$. As a consequence, we will have $v_t . e_t \geq 0$. On the other hand, we had $S_t . v_t \leq 0$, by the fact that $v_t$ is normal vector to $H_t$ on the other side of $S_t$. This implies that $\centerEllipse_t \notin \textrm{interior} (S_t)$. Moreover, because $\Tilde{H_t}$ is simply a shift of $H_t$ to make it pass through $\centerEllipse_t$, we can conclude $S_t \subseteq \Tilde{S_t}$. \qed
\end{proof}


\begin{corollary}
\label{cor: ellipse contains cone}
    In any inner while-loop, we always have $\dualcone_t \cap \ellipse_0 \subseteq \ellipse_t$.
\end{corollary}

\begin{proof}{\emph{Proof.}}
    By using \Cref{lemma: center is out of halfspace}, definitions of $\ellipse_{t+1}$ as well as $\dualcone_{t+1}$ in algorithm EEC (\ref{alg:Ellipsoid Exact Caratheodory}), and induction on $t$, we can write:
    \begin{align}
       \dualcone_{t+1} \cap \ellipse_0 = (\dualcone_{t} \cap S_t) \cap \ellipse_0 
        = (\dualcone_{t} \cap \ellipse_0) \cap S_t  
        \subseteq \ellipse_t \cap S_t 
        \subseteq \ellipse_t \cap \Tilde{S_t}
        \subseteq \ellipse_{t+1}
    \end{align}
    \qed
\end{proof}


Additionally, the following lemma tells us that the outer iteration is essentially reducing the dimension by restricting the search to lower and lower dimensional faces that the inner iteration may find, all of which still include the origin $\origin$ in them.

\begin{lemma}
\label{lemma: lower dimension faces include 0}
    Given $\mathfrak{h}=(h_1, h_2, ..., h_k)$ in any iteration, we have:
    $$\origin \in A_k,$$
    where $A_k$ is defined as in \Cref{def: Oracle_caratheodory} for Oracle($\mathfrak{h};P$).
\end{lemma}

\begin{proof}{\emph{Proof.}}
    We prove this lemma by induction on $k$, the length of $\mathfrak{h}$. If $k=0$ (i.e., the tuple is empty, e.g., at the beginning), we know $\origin \in P = A_0$ by assumption on $P$ and definition of $A_0$. Now suppose the property holds until some iteration with $\mathfrak{h}=(h_1, h_2, ..., h_k)$, and in the next outer iteration, we will have $\mathfrak{h} = \Tilde{\mathfrak{h}} = (h_1, h_2, ..., h_k, h_{k+1}=h_t)$, where $h_t$ corresponds to the last inner iteration before it stopped. It has to be the case that $\ellipse_{t+1} = \ellipse_{t}$, which only happens if the hyper plane $\Tilde{H_t}$ subsumes the entire $\ellipse_t$ rather than cutting it into half. Consequently, $v_t$ should be orthogonal to the $\ellipse_t$, and in particular to $h_t$, implying $h_t.v_t=0$. Now, note that due to induction hypothesis, we already know $\origin \in A_k$. Moreover, by definition of $v_t$, we know
    \begin{align}
        v_t \in A_{k+1} = \argmax_{u'\in A_{k}} h_{k+1}.u' \ \rightarrow \ \max_{u'\in A_{k}} h_{k+1}.u'=h_{k+1}.v_t = 0 = h_{k+1}.\origin \ \rightarrow \ \origin \in A_{k+1}.
    \end{align}
    This completes the induction proof.
\qed
\end{proof}



With these, we will now answer to the previous two questions via the following theorem.

\begin{theorem}
\label{thm: exact caratheodory alg}
    Algorithm EEC (\ref{alg:Ellipsoid Exact Caratheodory}) will terminate in polynomial time w.r.t. the size of the problem instance. Furthermore, if we denote by $\vertices_T$, the final set of points in $P$ output by the algorithm, we have:
    \begin{align}
        \origin \in \textrm{Conv}\{\vertices_T\}.
    \end{align}
\end{theorem}

\begin{proof}{\emph{Proof.}}
    To show that the algorithm terminates in polynomial time, notice that we are essentially running the ``ellipsoid algorithm" on $\ellipse_t$ during each round of the outer iteration, as $\ellipse_t \cap \Tilde{S_t}$ is a half ellipsoid. As such, we know that the volume of the ellipsoid will be geometrically shrinking, except only in the inner iterations that the hyper plane $\Tilde{H_t}$ subsumes the entire $\ellipse_t$ rather than cutting it into half, which only happens if the $\ellipse_t$ is in lower dimension and $v_t$ is orthogonal to it. If the latter case happens, as showed in \Cref{lemma: lower dimension faces include 0}, we can conclude that the origin is placed on the face induced by the sequence of directions $\Tilde{\mathfrak{h}}$ of that round, enabling us to (strictly) reduce the dimension of the face, in which we are searching over to cover $\origin$, for the rest of the outer iterations. Therefore, we can conclude that we can only have at most $\numaffine$ number of outer iterations, and for any of them, the inner iteration either gets to the case that $\ellipse_t=\{\origin\}$ in polynomial time (due to the geometric shrinkage)\footnote{Due to the known results for ``ellipsoid algorithm" running on a discrete space (due to numerical discritization), we know that after polynomial time w.r.t. the size of the bit-representation of the problem instance (which includes $N$, $\numaffine$, and the support of value distributions and costs), we eventually get to a point that only one (discrete) point will be left in $\ellipse_t$, which has to be the $\origin$.} or stops even sooner if $\ellipse_t=\ellipse_{t-1}$ and passes on to the next outer iteration, showing that the running time of the algorithm would be polynomial in the size of the input instance. 

    To prove that $\origin \in \textrm{Conv}\{\vertices_T\}$, suppose we are at the final round of the outer iteration. Denote by $H$ the hyper plane derived by projecting $\reals^\numaffine$ along with all directions in $\mathfrak{h} = (h_1, h_2, ..., h_k)$. Its not hard to verify that: i) $V_T \subset H$, ii) $\ellipse_0 \subset H$, and iii) $\origin \in A_k \subset H$. Now, due to the fact that the algorithm terminated at this round, we get that 
    $$\dualcone_T \cap \ellipse_0 \subseteq \ellipse_T=\{\origin\} \rightarrow \dualcone_T \cap H =\{\origin\} \rightarrow \cone_T = H 
    % \rightarrow \origin \in Convex\{-\vertices_T\} 
    \rightarrow \origin \in \textrm{Conv}\{\vertices_T\},$$
    completing the proof of the theorem.
    

    
    % XXX Both properties are pretty straightforward. The fact that the algorithm terminated means that $\dualcone_T \subseteq \ellipse_T=\{\origin\} \rightarrow \cone_T = \reals^\numaffine \rightarrow \origin \in Convex\{-\vertices_T\} \rightarrow \origin \in Convex\{\vertices_T\}$. As for the running time, we can say that at every iteration $t$, $\ellipse_t \cap \dualcone_{t+1}$ is, in fact, intersection of $\ellipse_t$ with a half-space that either does not contain $\centerEllipse_t$ or $\centerEllipse$ is on its border. Either way, $\ellipse_t \cap \dualcone_{t+1}$ would be at most half of $\ellipse_t$, and the rest of the running time analysis would be exactly the same as a typical ellipsoid algorithm. 
    \qed
\end{proof}

\begin{remark}
        To get further intuition on why $\origin \in \textrm{Conv}\{\vertices_T\}$, one can employ \Cref{lemma:covering} on the polytope $A_k = P \cap H$ to deduce that at any iteration $t$ during the inner loop, we know 
        $$\origin \in \textrm{Conv}\{\vertices_t, \argmaxCone_t \},$$
        where $\argmaxCone_t$ is defined as in \Cref{lemma:covering}, corresponding to the set $\vertices_t$ of points in $P$. Now, at a high-level, \Cref{alg:Ellipsoid Exact Caratheodory} is shrinking $\ellipse_t$, and consequently $\dualcone_t \cap \ellipse_0$, until a point that no non-zero direction will be left in it. This equivalently, enforces the $\argmaxCone_t$ to shrink until it becomes empty, and conversely enlarges $\cone_t$ to become the entire $\reals^\numaffine$, which results in
        $$\origin \in \textrm{Conv}\{\vertices_T, \argmaxCone_T \} = \textrm{Conv}\{\vertices_T\}.$$
\end{remark}







\subsection{Equality constrained problem}
\label{subsection: reduction of equality constrained to Caratheodory}

With our abstract problem being solved, let us get back to our main objective in this section, i.e., how we can exactly satisfy $\numaffine$ affine ex-ante constraints all at the same time. 
For now, suppose all of the constraints are equality constraints, due to simplicity of exposition. Later on, in \Cref{subsec: reduction of inequality to equality}, we will show how one can reduce a problem with multiple affine inequalities and equalities, to a problem that only have some equality constraints. 

Following the same approach as in the case of single affine constraint, the dual function (\ref{eq:dual_multiple}) derived by Lagrangifying all $\numaffine$ constraints will have same properties as before (such as being a piece-wise affine convex function) - now with $\LagVector \in \reals^\numaffine$.
\begin{align}
\label{eq:dual_multiple}
\DualLagrangeConst (\LagVector) \triangleq \max_{\policy \in \PolicySpace} ~\LagrangeConst (\pi;\LagVector)~.
\end{align}

Moreover, it continues to hold that a Gittin's index policy would be the maximizer solution for the Lagrangian adjusted version of the problem in \ref{eq:dual_multiple}, providing us with polynomial-time access to both the value and sub-gradients of $\DualLagrangeConst (\LagVector)$, as before. From standard convex optimization techniques (given access to the value and sub-gradients of $\DualLagrangeConst (\LagVector)$) we can efficiently find the vector of dual variables $\LagVector^*$ minimizing the dual function. However, it still remains a challenge on how to characterize the saddle point of this optimization problem - the randomized maximizer policy in \ref{eq:dual_multiple} for $\LagVector^*$ that achieves $\origin$ slack (as we assumed the constraints are all equality). This is especially challenging as the $\argmax$ set in \Cref{eq:dual_multiple} under $\LagVector^*$ may, in fact, contain exponential number of policies. Denote by $\mathfrak{I}$ the number of such best-response policies. For any $i \in [\mathfrak{I}]$, name the $i$-th policy as $\policy_i$, which arises from a particular tie-breaking rule $\tiebreak_i$ and associated with a particular slack vector $\slack_i \in \reals^\numaffine$. The goal here is to find an efficient way to select a handful of these policies that can provide us with $\origin$ slack (by randomizing over them). In other words, we would like to find a small subset of these policies $\{\policy_i\}_{i\in S}$, with $S \subseteq [\mathfrak{I}]$, such that:
$$\origin \in \textrm{Conv}\{\slack_i\}_{i \in S}.$$
Note that because we assumed the problem is feasible and $\LagVector^*$ is indeed the minimizer of $\DualLagrangeConst$, we already know that we can get $\origin$ slack by randomizing over all of these maximizer policies, i.e., 
$$\origin \in \textrm{Conv}\{\slack_i\}_{\forall i \in [\mathfrak{I}]}.$$

With this formulation of our problem and by setting all $\slack_i$ as the vertices of polytope $P$ in our previous discussion (i.e., $P\triangleq \textrm{Conv}\{\slack_i\}_{\forall i\in [\mathfrak{I}]}$), EEC (\ref{alg:Ellipsoid Exact Caratheodory}) will efficiently provides us our desired subset $S$, whose size would be polynomial w.r.t. the parameters of the problem, as shown by \Cref{thm: exact caratheodory alg}. Note that a single-Oracle (defined in \Cref{remark: Oracle Equivalency}) is nothing but finding the slacks for the policy with tie-breaking corresponding to the perturbation $\Tilde{h}_{\varepsilon}$.






\subsection{General constrained problem}
\label{subsec: reduction of inequality to equality}


We now show how to reduce a problem with some inequality constraints to a problem with only equality constraints. In particular, suppose our original problem has $\numaffine_n$ inequality and $\numaffine_e$ equality constraints ($\numaffine=\numaffine_n+\numaffine_e$). For any vector $v\in \reals^\numaffine$, we denote by $v[k]$, the $k$-th element of $v$. Suppose the first $\numaffine_n$ dimensions correspond to the slack of inequality constraints, and the rest indicate the slack for the equality constraints. Denote by $Q \subseteq \reals^\numaffine_+$ the set of all points $v$, that satisfy 
$\slack^*[k] = 0,\ \forall \numaffine_n < k \leq \numaffine$.

In the presence of inequality constraints, the goal of the problem is now to find a small subset of policies $\{\policy_i\}_{i\in S}$, with $S \subseteq [\mathfrak{I}]$, such that:
$$\textrm{Conv}\{\slack_i\}_{i \in S} \cap Q \neq \phi,$$
knowing that
$$P \cap Q \neq \phi,$$
where $P\triangleq \textrm{Conv}\{\slack_i\}_{\forall i\in [\mathfrak{I}]}$ as before.


To do this reduction, consider $\numaffine_n$ fictional policies, denoted by $\policy_{-i}, \forall i \in [\numaffine_n]$. For any $j \in [\numaffine_n]$, define the slack of $\policy_{-j}$ as follows:
\begin{align}  
    \slack_{-j}[k] \triangleq \begin{cases}
        -1, \quad & k=j,\\
        0, & k\neq j.
    \end{cases}
\end{align}
    
Now, let us define $\hat{P}\triangleq \textrm{Conv} \{ \{\slack_i\}_{\forall i \in [\mathfrak{I}] } \cup \{\slack_{-j}\}_{\forall j \in [\numaffine_n]} \}$.

Its easy to see the following holds on the relation of $P$ and $\hat{P}$:
$$P\cap Q \neq \phi  \quad \longleftrightarrow \quad \origin \in \hat{P}.$$
% \begin{lemma}
%     We have:
%     \begin{align}
%         P\cap Q \neq \phi  \quad \longleftrightarrow \quad \origin \in \hat{P}
%     \end{align}
% \end{lemma}

% \begin{proof}{\emph{Proof.}}
%     The proof is simple, and we defer it to the reader.
% \end{proof}

Moreover, note that given an Oracle($\mathfrak{h};P$), we can construct an Oracle($\mathfrak{h};\hat{P}$), by simply comparing all the $\numaffine_n$ vertices in $\{\slack_{-j}\}_{\forall j \in [\numaffine_n]}$ against the output of Oracle($\mathfrak{h};P$), for any $\mathfrak{h}$.

Putting all the pieces together, our reduction is as follows. We know $P\cap Q \neq \phi$, so we know $\origin \in \hat{P}$. Now, by using Oracle($\mathfrak{h};\hat{P}$), we can efficiently find a polynomial-sized subset of points $\vertices \subseteq {\hat{P}}$, such that $\origin \in \textrm{Conv}(\vertices)$. Nonetheless, we can partition $\vertices=\vertices_{\textrm{real}}\cup \vertices_{\textrm{fictional}}$, where $\vertices_{\textrm{real}} \subseteq P$ and $\vertices_{\textrm{fictional}} \subseteq \{\slack_{-j}\}_{\forall j \in [\numaffine_n]}$. Finally, its easy to verify that:
$$\textrm{Conv}(\vertices_{\textrm{real}}) \cap Q \neq \phi,$$
completing our reduction.

% \begin{lemma}
% \label{lemma: reduction of inequality to equality}
%     XXX
%     We highlight that if one can find an algorithm for \Cref{problem: exact caratheodory} 
% \end{lemma}

}

==> tex/app_copy_Exact_caratheodory.tex <==

{\color{brown}
\section{Multiple affine constraints: exact constrained optimal algorithm \& connections to algorithmic Carathéodory}
\label{sec:apx-caratheodory}


In this section, we provide a polynomial-time algorithm that extends our exact optimal solutions for the single affine constraint to the setting with $\numaffine>1$ number of such constraints.

Before going to the proof, we would like to state the following lemma:

\begin{lemma}
\label{lemma:covering}
    Consider a polytope $P \in \reals^\numaffine$ that includes the origin $\origin \in \reals^\numaffine$. Let $\vertices$ be a subset of the vertices of $P$. Denote by $\cone$ the "reverted'' cone of $\vertices$ (i.e., $Cone\{-\vertices\}$) and let $\dualcone$ be the dual cone of $\cone$. Lastly, let $\argmaxCone$ be the set of all vertices $u$ in $P$ for which there exist a direction $d$ in $\dualcone$ such that $d.u= \max_{u'\in P} d.u'$. Then, we have:
    $$\origin \in Convex\{\vertices, \argmaxCone \},$$
    where $Convex\{A,B\} \in \reals^\numaffine$ is the convex combination of all points in $A\cup B$.
\end{lemma}

\begin{proof}{\emph{Proof.}}
    Suppose $\origin \notin Convex\{\vertices\}$, as otherwise we are clearly done. This implies that $\cone \cap Convex\{\vertices\} = \phi$. With this in mind, its not hard to see that:
    \begin{align}
    \label{eq:covering_equivalency}
        \origin \in Convex\{\vertices, \argmaxCone \} \iff \cone \cap Convex\{\argmaxCone\} \neq \phi.
    \end{align}
    Additionally, we can assume that both $\vertices$ and $\argmaxCone$ are non-empty, as otherwise we have:
    \begin{itemize}
        \item if $\vertices=\phi$: then $\cone=\{\origin\} \rightarrow \dualcone=\reals^\numaffine \rightarrow \argmaxCone=P \rightarrow \origin \in P = Convex\{\argmaxCone\}$, and we are done.
        \item if $\argmaxCone=\phi$: then it means there was no direction in $\dualcone$, so $\dualcone = \{\origin\} \rightarrow \cone = \reals^\numaffine \rightarrow \origin \in Convex\{-\vertices\} \rightarrow \origin \in Convex\{\vertices\}$, and we are done.
    \end{itemize}
    Now, we prove RHS of \Cref{eq:covering_equivalency} by contradiction. Suppose $\cone \cap Convex\{\argmaxCone\} = \phi$, then there exists a strict separating hyperplane $H$ that separates $\cone$ and $Convex\{\argmaxCone\}$, as both of them are non-empty closed convex sets and $Convex\{\argmaxCone\}$ is compact. With out loss of generality we can assume that $H$ passes through $\origin$ (the vertex of $\cone$. Let $h$ be the normal vector of $H$, pointing to the side of $H$ that includes $\cone$. We should have $h \in \dualcone$. Now, define $u \triangleq \argmax_{u'\in P} h.u'$, then we should have:
    \begin{equation}
    \left.
    \begin{aligned}
    & \bullet \quad h \in \dualcone \quad \rightarrow \quad u \in U \\
    & \bullet \quad \origin \in P \quad \rightarrow \quad u.h \geq 0.h = 0 \\
    & \bullet \quad \textrm{$U$ is on the other side of H as h} \quad \rightarrow \quad 0 > U.h
    \end{aligned}
    \quad\right\rbrace \rightarrow \bot \quad (\textrm{contradiction!})
    \end{equation}
\qed
\end{proof}

Now that we have proved \Cref{lemma:covering}, we will provide our polynomial time algorithm, EEC (\ref{alg:Ellipsoid Exact Caratheodory}), to recover a subset $\vertices$ of the vertices of $P$ that cover $\origin$, i.e., $\origin \in Convex\{\vertices\}$ - assuming that we can solve $\argmax_{u'\in P} h.u'$ efficiently for any arbitrary direction $h$.



\begin{algorithm}
\caption{Ellipsoid Exact Caratheodory (EEC)}
\label{alg:Ellipsoid Exact Caratheodory}
    \SetKwInOut{Input}{input}
    \SetKwInOut{Output}{output}
\Input{Oracle solving $v=\argmax_{u'\in P} h.u'$ for any $h$.}

At $t=0$: Let $\ellipse_0$ be the unit ball in $\reals^\numaffine$, and let $\centerEllipse_0=\origin$ be its center. Let $\vertices_0=\phi$.

% Choose an arbitrary direction $h_0$ and find $v_0=\argmax_{u'\in P} h_0.u'$. Set $\vertices_0=\{v_0\}$, and construct $\cone_0, \dualcone_0$ based on $\vertices_0$. Lastly, have in mind $\argmaxCone_0$ based on $\dualcone_0$ (without characterizing it).
 
\vspace{1mm}

\While{$\ellipse_t \neq \{\origin\}$}{
\vspace{1mm}
Choose $h_t := \centerEllipse_t$, the center of ellipsoid $\ellipse_t$. If $\origin = \centerEllipse_t$, then choose an arbitrary direction $h_t$.

Find $v_t=\argmax_{u'\in P} h_t.u'$ and set $\vertices_{t+1}:=\vertices_t \cup v_t$. 

Define $H_t$ as the linear space orthogonal to $v_t$  and let $S_t$ be the half space of $H_t$ not including $v_t$. In other words, $H_t . v_t =0$ and $S_t . v_t \leq 0$.


Let $\Tilde{H_t}$ be the hyper plane parallel to $H_t$ and passing through $\centerEllipse_t$, and $\Tilde{S_t}$ be its half space.

Construct $\cone_{t+1} := Cone\{-\vertices_{t+1}\}=Cone\{\cone_{t}, - v_t\}$, $\dualcone_{t+1} := DualCone\{\cone_{t+1}\} = \dualcone_{t} \cap S_t$.


Find $\ellipse_{t+1}$ as the ellipsoid constructed in the ``ellipsoid algorithm" containing $\ellipse_t \cap \Tilde{S_t}$.

$t+=1$.
}

\vspace{2mm}

\Output{set $\vertices_t$ of final nodes recovered.}
\end{algorithm}


We will now show that why the output of this algorithm can cover $\origin$ and why it will terminate in polynomial time, but before that we state the following lemma and its important corollary:
\begin{lemma}
\label{lemma: center is out of halfspace}
    We always have $\centerEllipse_t \notin \textrm{interior} (S_t)$. Accordingly, $S_t \subseteq \Tilde{S_t}$.
\end{lemma}

\begin{proof}{\emph{Proof}}
    First of all, if $\centerEllipse_t=\origin$, then we have $H_t=\Tilde{H_t}$ and $S_t=\Tilde{S_t}$. Else, note that, in \Cref{alg:Ellipsoid Exact Caratheodory}, we set the miximization direction $h_t$ equal to $\centerEllipse_t$. As a consequence, we will have $v_t . e_t \geq 0$. On the other hand, we had $S_t . v_t \leq 0$, by definition. This implies that $\centerEllipse_t \notin \textrm{interior} (S_t)$. Moreover, because $\Tilde{H_t}$ is simply a shift of $H_t$ to make it pass through $\centerEllipse_t$, we can conclude $S_t \subseteq \Tilde{S_t}$. \qed
\end{proof}


\begin{corollary}
\label{cor: ellipse contains cone}
    We always have $\dualcone_t \cap \ellipse_0 \subseteq \ellipse_t$.
\end{corollary}

\begin{proof}{\emph{Proof}}
    Straightforward by using \Cref{lemma: center is out of halfspace}, definitions of $\ellipse_{t+1}$ as well as $\dualcone_{t}$ in \Cref{alg:Ellipsoid Exact Caratheodory}, and induction.  \qed
\end{proof}
    

\begin{theorem}
    \Cref{alg:Ellipsoid Exact Caratheodory} will terminate in polynomial time w.r.t. the size of the problem instance. Furthermore, if we denote by $\vertices_T$, the set of vertices recovered by the algorithm, we have:
    \begin{align}
        \origin \in Convex\{\vertices_T\}.
    \end{align}
\end{theorem}

\begin{proof}{\emph{Proof}}
    To show that the algorithm terminates in polynomial time, notice that we are essentially running the ``ellipsoid algorithm" on $\ellipse_t$, as $\ellipse_t \cap \Tilde{S_t}$ is a half ellipsoid passing through its center. As such, we know that the volume of the ellipsoid is geometrically shrinking. Moreover, notice that by \Cref{cor: ellipse contains cone}, we know that it always contains $\dualcone_t \cap \ellipse_0$. This means that $\dualcone_t \cap \ellipse_0$ must shrink geometrically. Due to the known results for ``ellipsoid algorithm" running on a discrete space (due to numerical discritization), we know that after polynomial time w.r.t. the size of the bit-representation of the problem instance (which includes $N$, $\numaffine$, and the support of value distributions and costs), we get to the point that only one (discrete) point will be left in $\ellipse_t$ (and thus $\dualcone_t \cap \ellipse_0$) and the center of $\ellipse_t$ ($\centerEllipse_t$) would lie on 
    
    XXX Both properties are pretty straightforward. The fact that the algorithm terminated means that $\dualcone_T \subseteq \ellipse_T=\{\origin\} \rightarrow \cone_T = \reals^\numaffine \rightarrow \origin \in Convex\{-\vertices_T\} \rightarrow \origin \in Convex\{\vertices_T\}$. As for the running time, we can say that at every iteration $t$, $\ellipse_t \cap \dualcone_{t+1}$ is, in fact, intersection of $\ellipse_t$ with a half-space that either does not contain $\centerEllipse_t$ or $\centerEllipse$ is on its border. Either way, $\ellipse_t \cap \dualcone_{t+1}$ would be at most half of $\ellipse_t$, and the rest of the running time analysis would be exactly the same as a typical ellipsoid algorithm. \qed
\end{proof}


With this, let us go back to our main objective in this section, i.e., how we can exactly satisfy $\numaffine$ affine ex-ante constraints all at the same time. Following the same approach as in the case of single affine constraint, the dual function (\ref{eq:dual_multiple}) derived by Lagrangifying all $\numaffine$ constraints will have same properties as before (such as being a piece-wise affine convex function) - now with $\LagVector \in \reals^\numaffine$.
\begin{align}
\label{eq:dual_multiple}
\DualLagrangeConst (\LagVector) \triangleq \max_{\policy \in \PolicySpace} ~\LagrangeConst (\pi;\LagVector)~.
\end{align}

 Moreover, it continues to hold that a Gittin's index policy would be the maximizer solution for the Lagrangian adjusted version of the problem in \ref{eq:dual_multiple}, providing us with polynomial-time access to both the value and sub gradients of $\DualLagrangeConst (\LagVector)$, as before. From standard convex optimization techniques (given access to the value and subgradients of $\DualLagrangeConst (\LagVector)$) we can efficiently find the vector of dual variables $\LagVector^*$ minimizing the dual function. However, it still remains a challenge on how to characterize the saddle point of this optimization problem - the randomized maximizer policy in \ref{eq:dual_multiple} for $\LagVector^*$ that achieves $\origin$ slack. This is especially challenging as the $\argmax$ set may, in fact, contain exponential number of policies $\policy_i$, each arising from a particular tie-breaking rule $\tiebreak_i$ and associated with a particular $\numaffine$-dim vector of slack $\slack_i$. The goal here is to find an efficient way to select a handful of these policies that can provide us with $\origin$ slack (by randomizing over them). In other words, we would like to find a small subset of these policies $\{\policy_i\}_{i\in S}$, such that:
 $$\origin \in Convex\{\slack_i\}_{i \in S}.$$
 Note that because we assumed the problem is feasible and $\LagVector^*$ is indeed the minimizer of $\DualLagrangeConst$, we already know that we can get $\origin$ slack by randomizing over all of these maximizer policies, i.e., 
 $$\origin \in Convex\{\slack_i\}_{\forall i}.$$

With this formulation of our problem and by setting all $\slack_i$ as the vertices of polytope $P$ in our previous discussion, \Cref{alg:Ellipsoid Exact Caratheodory} will provide us the desired subset $S$, whose size would be polynomial w.r.t. the parameters of the problem.

}

==> tex/app_fairness-examples.tex <==
\section {More Examples of Ex-ante Fairness via Affine and Convex Constraints}
\label{apx:fairness-examples}

In this appendix we will mention a couple of different ways one can implement some notions of fairness, using our "general" fairness constraints that introduced in \Cref{sec:JMS-setting}.

\RN{@Mohammad Reza Task 3: at some point I would like you to write some examples of incorporating fairness constraints using our affine and convex constraints in this appendix section. For example, we discussed having multiple partitioning of the society into demographic groups, e.g., along race, gender, wealth, and then using a weighted sum of negative entropy of utilities for each group as a function that measures "fairness". It would be helpful to add similar examples in this appendix section.}
\begin{enumerate}
    \item 
\end{enumerate}

==> tex/app_rawpandora.tex <==

\section{MR Appendix raw material ...}


















==> tex/app_taxation.tex <==
\section{Delegated Pandora's Box: Demographic Parity through Taxation}

\label{sec:tax}


==> tex/conclusion-short.tex <==
%\vspace{-4mm}
\section{Conclusion and Future Directions}
\label{sec:conclusion}
\revcolor{We initiate the study of adding ex-ante constraints to Markovian sequential search with costly information acquisition. Our study is motivated by the rise of algorithmic hiring and the interest in improving measures of diversity and inclusion. We encode many of such measures as general ex-ante constraints and design optimal constrained policies (or nearly optimal and near feasible ones) for the underlying search processes. We view our work as a building block for understanding the efficiency–fairness trade-off, a direction we plan to pursue.

Although we focus on ex-ante fairness---natural in settings where the search repeats many times (e.g., pre-employment screening)---studying ex-post fairness across different stages of a single, high-stakes search is another promising direction. For instance, how can we ensure an ex-post balance in interviews for a top executive hire? Additionally, many search processes are \emph{delegated} in principal–agent frameworks, raising questions about how to induce fairness when only the principal values it. 

% Also, a future direction, ex-ante constraints can capture several operational limitations and be studied in other applications of sequential search beyond hiring, such as facility location with costly inspection (e.g., for placing windmills in different locations).


Finally, we adopt the classic Pandora's box assumptions of known, independent reward distributions. Recent work has begun to relax these assumptions—e.g., by considering unknown distributions or correlated boxes—albeit without fairness considerations \citep{chawla2020pandora, gatmiry2022bandit}. Revisiting these richer settings with well-defined notions of fairness is an appealing avenue for future research.}



% Our work can be used as a building block to understand and characterize the inherent trade-off between efficiency and various fairness measures, which is the research direction that we plan to pursue. Further, here we focus on notions of ex-ante fairness which are natural and motivated in contexts where the search process repeats over many instantiations, e.g., an algorithm is repeatedly used for pre-employment selection (see \citet{raghavan2020mitigating} for discussions and examples). Studying notions of {\em ex-post} fairness in various stages of the search process can be relevant and is a fruitful research direction. For example, when searching for a top executive---a high-stakes and rare search process---how to design an optimal policy (or an approximation of it) that ensures that the ex-post number of inspected boxes in the Pandora's box problem interviewed candidates (i.e., inspected boxes in the Pandora's problem) is balanced across demographic groups?  
% Additionally, in practice, many search processes are {\em delegated}, thus studied in principal-agent frameworks. What if only the principal cares about fairness? 
% How to induce fairness in delegated search? 
% Finally, in studying the Pandora's box problem and its variants,  
% following the classic setting, we assume that the reward of boxes are independent and their distributions are known. Relaxing both of these assumptions is practically well-motivated. 
% As mentioned in \Cref{sec:further-related-work},  a few recent papers study more realistic settings by relaxing these assumptions albeit without regard to fairness considerations \citep{chawla2020pandora, gatmiry2022bandit}. Revisiting these richer settings under well-defined notions of fairness is an interesting direction for future research.









==> tex/intro-before-revision.tex <==

% \RN{To do:
% \begin{itemize}
% \item MReza: Reading the whole paper and making sure everything is in place.
% \item MReza: I am still running the codes. Once I upload the new figures, I will let you know. Then please update all the figures (main and appendix) in the overleaf.
% \item Rad: Take a pass over further related work, abstract, and conclusions. Make them consistent with the current numerical.
% \item \sout{MReza: I left you two comments regarding the proof of Thm 2 in the appendix. Please address them.}
% \item \sout{MReza: make sure all the pointer to EC are correct and it is referred to as "appendix".}
%  \item \sout{MReza : Revising the refinement 
%  subsection in the main body.}
%  \item \sout{MReza: add a citation to the source for Fig 3 part c (the skill distribution). Use ChatGPT to create the bib entry!}
%     \item \sout{Rad : Taking a pass over numerical in the appendix and making it consistent with main body}
%     \item \sout{MReza :  Reading numerical in the main body and add comments/revising.}
%     \item \sout{Rad, MReza : Making sure all the plots and codes are giving us the final plots and then plotting everything again and have all the final plots ready.}
%     \item \sout{Rad : Taking a pass over intro and applying all the comments}
%     \item \sout{MReza : double-checking the proofs of the refinement section and making sure it is all correct and consistent with main}
%     \item \sout{Rad : pass through the refinement proof after revising the refinement section + take a pass over refinement in main}
%     \item \sout{Rad : Updating intro and add stuff from new numerical} 
%     \item \sout{Rad: Take a final pass over numerical section after MReza.}
% \end{itemize}
% }
\section{Introduction}
\label{sec:intro}

Decisions that profoundly influence the course of an individual's life, such as those related to hiring and admissions, have historically exhibited biases against specific demographic groups. For example, \citet{bertrand2004emily} found that applicants with typically African-American names received fewer interview calls than those with traditionally white names, illustrating the deeply entrenched nature of such biases. This has resulted in persistent disparities in diversity and representation, which, in the long run, can lead to undesirable economic and societal outcomes in these domains~\citep{becker2010economics}. Despite continuing efforts to rectify these disparities, the progress has been stagnant. The meta-analysis by \citet{quillian2017meta} underscores this concern, indicating that racial discrimination in hiring practices has seen little improvement in recent decades. 

The rise of algorithmic hiring, that is, the practice of using data-driven algorithms for (possibly sequential) search and selection among candidates, offers a promising avenue to disrupt this pattern. These algorithms take advantage of computational resources and, therefore, are typically faster and more efficient than their human counterparts; furthermore, they do not introduce or perpetuate explicit bias by design. However, there remains a risk of implicit marginalization by these algorithms arising from the potential biases present within the ``input data'' that inform their decisions. Consider the standardized tests used in college admissions as an example. There exists a systematic disparity in scores among students of different socioeconomic backgrounds, largely attributed to the variability in the quality of test preparations conducted by schools~\citep{sackett2012role, kleinberg2018algorithmic}. Furthermore,  regardless of decision-making agents --- be it algorithms or humans --- marginalization can be influenced by other factors at play; for example, underprivileged individuals may not even have the means or access to apply for certain positions or institutions, or cannot afford tuition or application expenses for certain schools, and therefore remain underrepresented ~\citep{gaddis2013influence,chetty2020income}.
These and similar concerns have spurred the growth of automated hiring tools and platforms that aim to \emph{proactively} mitigate various forms of bias and promote equity, diversity, and inclusion by calibrating outcomes~\citep{garr2019diversity, raghavan2020mitigating}. 


A school of thought to achieve socially desirable outcomes in the presence of such disparities is to influence the algorithm's decisions by imposing certain \emph{socially aware constraints} on its induced statistical behavior. These constraints, which are typically held on average and, therefore, are called \emph{ex-ante} constraints, can capture various measures of fairness and diversity in the underlying decision processes. The sub-field of algorithmic fairness in computer science introduced and studied several such notions in machine learning problems such as classification and regression and provided means of satisfying those on-average constraints; see the discussion in \citet{kleinberg2018algorithmic}. 

However, search and selection processes can involve operational intricacies, which makes the underlying problem fundamentally different from classification or regression. These include capacity constraints, costly information acquisition through inspection, and the sequential nature of some selection processes. 
As such, the overarching goal of our work is to take the first step toward complementing the algorithmic fairness literature by taking into account operational aspects of search and selection processes while imposing socially aware constraints. 

More concretely,  we focus on a general framework to model a large class of sequential search and selection processes that we call {\em Markovian search}. Roughly speaking, a Markovian search models a stateful search process where each candidate transitions across different states (e.g., uninspected, inspected, selected, etc.) according to a Markov chain.~\footnote{We defer the formal definition to \Cref{sec:general}.} Transitions occur when the decision maker takes an action (often costly) for a candidate, such as inspecting or selecting them. For such a setting, our objective is to understand the intricate interplay between operational components and socially aware constraints from a computational perspective. In particular, our main research question is the following:

\smallskip
\begin{displayquote}
{\em For a Markovian search process, how to formalize various notions of socially aware ex-ante constraints and how to 
design (and efficiently compute) optimal or near-optimal policies satisfying these constraints?} 
\end{displayquote}
\smallskip

Before providing an overview of our work, we emphasize that we do not take a stand in favor or against any of these constraints, nor do we comment on the ongoing legal discussion around some of them (for example, see the discussion in \cite{ho2020affirmative} on legal grounds of algorithmic fairness). Instead, our work sheds light on how imposing various constraints poses new computational challenges and changes the structure of the optimal policy. An important managerial insight of our work is that an algorithmic decision maker can devise near-optimal policies that respect a rich set of socially aware constraints through carefully designed randomization and simple, often interpretable, modifications of the original (unconstrained) problem. 

\smallskip
% \VM{The above is meant to replace the next two parags;  }
% They can also help employ operational levers, such as subsidy allocations given an average budget, in a smart way to equalize the opportunity landscape.
% Subscribing to this school of thought, satisfying these ex ante constraints has an intricate interplay with operational constraints such as sequential aspect of several search processes, resource limitations, costly acquisition of information, and inherent complexity of many of these search processes (e.g., multiple stage of interview); therefore, it poses significant computational challenges for a socially conscious algorithmic decision maker in these contexts. Motivated by this, we study general models of sequential search and selection processes subject to various forms of ex-ante constraints on the outcome distribution of the resulting algorithms. Our overarching research question is the following:

% \smallskip
% \begin{displayquote}
% {\em In a Markovian environment with costly acquisition of information about candidates, how to design (and efficiently compute) optimal or near-optimal sequential search and selection policies satisfying a general notion of socially aware ex-ante constraints?} 
% \end{displayquote}
% \smallskip




% \VM{Ok for now, but we need to shorten it.}
\noindent{\textbf{Basic Model -- Pandora's Box (\Cref{sec:pandora}).} Toward answering the above question, we first augment the classic model of sequential search known as the {\em Pandora's box problem}~\citep{weitzman1979optimal} with a simple form of ex-ante constraint, which turns out to be critical in our applications. In the original model, a decision maker is presented with a set of alternatives (or boxes), each of which is associated with an independent stochastic reward --- which should be thought of as the quality of the corresponding candidate. The decision maker's goal is to select a subset of these boxes smaller than a given capacity. A priori, she only has distributional knowledge about the rewards. However, if she inspects a box at a known cost, e.g., by interviewing the candidate, the box opens and its actual reward is observed. Any open box can be selected at any time if there exists available capacity. Naturally, the main goal is to find an optimal policy to maximize the net utility. This model captures the tension between stopping the search (to avoid additional inspection costs) and continuing (to look for better alternatives). Remarkably, as shown in \cite{weitzman1979optimal} --- and later extended to multiple selections in \cite{singla2018price} --- the optimal unconstrained policy is an \emph{index-based policy} that adaptively keeps track of a simple polynomial-time computable index for each box and greedily inspects (selects) the unopened (open) box with highest nonnegative index until it runs out of capacity or all remaining indices are negative. We should also note that these indices are essentially \emph{Gittins indices}~\citep{gittins1979bandit} adapted to the Pandora's box problem.



Our variant of Pandora's box involves an additional constraint: Taking into account the vector of selection and inspection probabilities of different boxes, we impose an affine constraint on this vector. We then ask, given this constraint, how to characterize (and compute) the optimal constrained policy. As a concrete example, consider boxes that belong to one of the two demographic groups and let the decision maker know these attributions upfront. Aware of implicit biases in reward distributions or cost disparities between these two demographic groups, the decision maker imposes {\em demographic parity}, namely equalizing the expected number of selections (or inspections) between the two groups. Alternatively, if a group represents a minority, the decision maker could set an average \emph{ quota} to enhance diversity, in the spirit of the widely practiced $4/5$ rule~\citep{raghavan2020mitigating}, ensuring that the expected number of selections (resp. inspections) from the minority group is at least a certain fraction of the expected number of total selections (resp. inspections). Additionally, in scenarios where certain candidates are underprivileged and cannot afford associated expenses for either selection (e.g. college tuition) or inspection (e.g. application costs),
% \VM{do we mean interview costs? also, aren't those paid by the decision maker? we should be careful here, o/w people may get the impression that the boxes pay the cost $c$ not the decision maker...}
% \MA{Dear Vahideh, here we talk about the budget constraint, when the decision maker has some budget to waive application fee/tuition for poor people, and thus it can essentially include them in its search. We are kinda assuming the bigger pool is known somehow, and we can subsidize some part of inspection costs by using that exogenous budget. Say, everyone fills out the application form, under regular setting anyone who don't pay an application fee, won't be considered for an interview, but with the help of this budget, they might still be considered for interview if their CV and value distribution looks good.}
the decision maker may operate under an average \emph{budget} constraint to subsidize these expenses.  Lastly, to truly mitigate disparities and avoid superficial token selections or inspections, the aforementioned constraints could be refined to focus only on alternatives with high enough quality or top quantiles of each box's reward distribution. Our general class of ex-ante affine constraints, formally defined in \Cref{sec:single-affine}, and its refinement with different coefficients for different rewards, formally defined in \Cref{sec:quantile-constraint}, include all these scenarios and beyond.

 
As our first main result, we characterize the optimal constrained policy that satisfies the ex-ante affine constraint \emph{exactly}; see \Cref{thm:const} for the basic version and \Cref{prop:general-constraint} for the refined version. We show that the optimal constrained policy, which is called \emph{Randomized Dual-adjusted Index Policy} (RDIP), has a remarkably simple structure (\Cref{alg:const}): It randomizes between at most two deterministic index-based  policies, both relying on the same set of indices, and they only differ in tie-breaking decisions. Furthermore, these indices are simple adjustments to the Gittins indices for the original model. Generally known to be brittle, it is intriguing that adding our general affine constraint does not break the optimality of index-based policies. The reason behind this is the existence of a relaxed Lagrange dual function for the constrained problem that can be viewed as an unconstrained Pandora's box problem but for an {\em adjusted instance}. Later, we will build on this observation in our general model. 



From a computational perspective, we also show that both the adjusted indices and the two relevant tie-breaking rules are polynomial-time computable, despite the fact that there are potentially exponentially many tie-breaking rules for an adjusted index-based policy. In fact, we show that the ``correct'' adjustment can be computed by solving a certain convex program related to the relaxed Lagrange dual function. Moreover, we show that our tie-breaking rules have an intuitive closed-form characterization and correspond to two perturbations of the correctly adjusted index-based policy that try to maximize the slack in positive and negative directions, respectively; see \Cref{def:tie:extreme} for the closed forms of these tie-breaking rules under the basic version of our constraint and \Cref{def:refined-ext-tie} under the refined version of our constraint.

These adjustments have interesting economic interpretations in our application: Taking demographic parity in selection as an example, it suffices to uniformly shift the {\em rewards} of all members of each group by the same amount but in opposite directions for each group, leaving the inspection costs unchanged. Interestingly, such a uniform adjustment in rewards implies that the order of search among the members of each group remains the same as in a setting where we conduct searches separately for each group. Preserving {\em within group} order is generally desirable, as discussed in the context of algorithmic fairness (see \citet{kleinberg2018algorithmic} and references therein). As another example, to satisfy the inspection quota constraint (say among candidates whose quality is higher than a certain threshold to avoid token interviews), we may
% \MAdelete{uniformly} \MA{not that the costs would be proportional to probability of each candidate's value be larger than the threshold. I think its better not to use quantile-base threshold, and say value-base threshold, especially if we want to confront tokenism} 
shift the \emph{inspection costs} of all candidates in the minority group downward~\footnote{but not uniformly, in fact, proportional to the probability of each candidate's quality being higher than the threshold.}, and proportionally shift that of all candidates in the other group upward, while keeping the rewards unchanged. In contrast to parity in selection, such an adjustment may change the order within each group, implying that quota in inspection may come at the expense of distorting within-group orders (see the related discussion in \Cref{sec:lagrangian-pandora} and \Cref{sec:insights-dem-parity} for further elaboration).
 
 
\smallskip


\noindent\textbf{General Model -- Joint Markov Scheduling (\Cref{sec:general}).} While the Pandora's box problem has served as a cornerstone for the study of sequential search problems, realistically,  hiring decisions involve richer search processes. We present one such example in the following. 

\smallskip
\begin{example}[Multi-stage Search with Rejection]
\label{ex:reject}
The hiring process for various jobs involves two stages of inspection. The first, a low-cost stage, might take the form of a phone interview and provide basic pass/fail information about a candidate. The second stage is more costly, involving an onsite visit, and offers a comprehensive evaluation of the candidate's quality. At each point, the hiring firm has three choices: conduct the first stage for a new candidate, proceed to the second stage for a candidate who passed the first, or make an offer, which itself has associated costs, to a candidate who has passed both stages. The chosen candidate may decline the offer, which happens with a certain probability, allowing the decision-maker to resume the search.
\end{example}
\smallskip

This is just one example of a ``stateful'' search process in which the underlying status of a box (modeling a candidate) can evolve each time the decision-maker interacts with it. As a result, the search process can depend on the current observable \emph{state} of each box. This state encodes the box's status and the cost of inspecting it (or the realized reward of selecting this box if it is already opened). The stateful nature of these applications gives rise to highly complex policies that may suffer from various types of biases in different stages of the search process or their final outcomes. Motivated by this, in \Cref{sec:general}, we study how to incorporate a reasonably \emph{general class of ex-ante constraints} in such settings. Going beyond the basic Pandora's box model and the particular notion of single affine constraint,  we model a general Markovian sequential search process as a \emph{joint Markov scheduling (JMS) problem} --- which has been extensively studied in the literature~\citep{gittins1979bandit,dumitriu2003playing} --- under our general ex-ante constraints, which we detail later.


A Markovian sequential search problem can be captured using JMS by modeling each box as an {\em absorbing Markov chain (MC)} with terminal states. 
Each time the decision maker interacts with a box, the corresponding MC undergoes a stochastic state transition. A box is ``selected'' when its MC transitions to one of its terminal states. Each state is associated with a reward, often negative for non-terminal states (capturing costs) and positive for the terminal ones (encoding potential gain from selection).\footnote{As we see later in \Cref{sec:optimal-JMS-arbitrary}, for reasons related to satisfying our socially aware constraints by adjusting the rewards, we need to go beyond this setting by considering instances with \emph{arbitrary} positive or negative state rewards.}
The search process entails choosing --- which is the analog of inspecting --- one of these MCs sequentially at each time, and terminating when a subset of boxes with size equal to the capacity is selected (or terminating early by leaving the remaining capacity unallocated). In the original unconstrained model, the decision maker's goal is to sequentially and adaptively choose/inspect the MCs to maximize her expected net reward until termination. We formally introduce this setting in \Cref{sec:JMS-setting}. Furthermore, in Figures \ref{fig:pandora-jms} (resp.  \ref{fig:MC-hiring}), we illustrate the JMS representation for a toy instance of Pandora's box problem (resp. \Cref{ex:reject}). 

%\VM{my suggestion: switch the order in fig 1 and then also explain Pandora a bit more. There is nice footnote in the next parag. that is currently commented out. I think we can just condense this and put in it the caption?}     



%CFN: To model the utilities, each state is associated with a reward, which is usually assumed to be negative for non-terminal states as a cost should be paid for inspecting an arm, and positive for terminal states  as a value is made from selecting an arm.\footnote{As we see later in \Cref{sec:optimal-JMS-arbitrary}, for reasons related to incorporating fairness by adjusting the rewards, we need to go beyond this setting and consider problem instances with \emph{arbitrary} positive or negative state rewards.} The goal of the decision maker is to adaptively select and interact with these MCs to maximize the total collected rewards until one of the chains reaches a terminal state (and hence be selected).  Importantly, this model also subsumes the Pandora's box model of \cite{weitzman1979optimal} as a special case.\footnote{To see this, for each box $i\in[n]$ consider a Markov reward process with one initial state ``not opened'' with reward $-c_i$, one state for each possible value realization $v_i\in\values_i$ with reward $v_i$ (and state transition probability of $F_i(v_i)$ from the initial state), and one terminal state with reward $0$.} 

Equipped with the JMS framework, we incorporate notions of socially aware constraints beyond a single affine ex-ante constraint. We allow any arbitrary number of general \emph{affine or convex constraints over the vector of ex-ante outcomes} of the search process. At a high level, for a given policy, we focus on the vector of the expected visit numbers of each state of each box, and we impose our constraints on such a vector.  
Our approach is flexible enough to capture various notions of fairness at the group-level and individual level considered in the literature, as well as additional operational constraints on average.
For example, in the multi-stage search described in \Cref{ex:reject} we can simultaneously capture an average quota constraint on final selections, together with an expected budget constraint on the number of offers made. Additionally, in contexts such as hiring, advancing in the search process may come with benefits for the candidates (e.g., gaining experience or visibility) even if they are not selected. Modeling this benefit as a utility function for each box that depends on its ex-ante outcomes, the decision maker may want to maintain equity in terms of these utilities among similar individuals.  Our framework can also capture this by ensuring that nonlinear egalitarian welfare measures such as Nash social welfare or minimum utility are higher than a certain threshold through a convex ex-ante socially aware constraint~\citep{kaneko1979nash,dwork2012fairness}. We also formalize our general constraints and the corresponding constrained problem in \Cref{sec:JMS-setting}.  

As our second main result, we present a fully polynomial-time approximation scheme (FPTAS), called {\em Generalized Randomized Dual-adjusted Index Policy} (G-RDIP), which efficiently computes an almost feasible and optimal policy. Concretely, given positive constants $\varepsilon$ and $\delta$, we find a randomized policy with an expected objective value within an additive $\varepsilon$ error of the optimal constrained solution that satisfies all the constraints within an additive error of $\delta$, with a polynomial running time in $\tfrac{1}{\varepsilon}$, $\tfrac{1}{\delta}$, and the size of the input instance (see \Cref{alg:RAI} and \Cref{thm:RAI}). Similar to \Cref{sec:pandora}, an essential building block of our algorithm design is the optimal solution for the unconstrained JMS problem. Prior work has shown that JMS admits a Gittins index-based optimal policy under certain assumptions on the state rewards~\citep{gittins1979bandit,dumitriu2003playing}. In \Cref{sec:optimal-JMS-arbitrary}, we refine these results to show that the index-based structure of the optimal policy can be preserved even for arbitrary state rewards through a pre-processing step (see \Cref{thm:JMS-optimal-reduction-informal}). 

The above refinement is necessitated by our key observation that the Lagrangian relaxation of the optimal constrained problem can be viewed as an unconstrained JMS with a particular regularizer in the objective. With only affine constraints, similar to \Cref{sec:pandora}, this new problem is indeed an unconstrained JMS under an adjusted instance. However, in the presence of convex constraints, the objective function of the new JMS will no longer remain linear in the ex-ante outcome vector --- and hence not only it is not associated with an adjusted instance, it is not even clear whether there exists a polynomial-time optimizer for this objective. To overcome this challenge, we further relax the Lagrangian dual function by applying Fenchel's weak duality on the concave terms (we review the basics of this machinery in Appendix~\ref{sec:convex}), which results in a relaxation that is still non-linear but this time bilinear with respect to the two sets of dual variables: those corresponding to constraints and those corresponding to Fenchel duality. Taking a game-theoretic view for solving max-min saddle-point problems, we aim to solve the zero-sum game between the primal player (decision maker, who picks a randomized policy) and the dual player (who picks these two sets of duals) in this relaxed Lagrangian game. Our policy G-RDIP not only finds an approximate equilibrium for this game, but also provides a certificate that this relaxed game is tight up to small additive errors compared to the original game. 
%CEC \VM{should we say more and talk about co-linearity of $\mu$ and $\beta$? I'd say no.}

To show the above claim, our policy uses a simple two-layer iterative learning algorithm that crucially exploits our problem's structure. We provide an overview of our design in \Cref{sec:RAI}. The resulting algorithm randomizes among polynomially many deterministic index-based policies, each of which is an optimal policy for an adjusted JMS instance with adjustments based on the dual estimates of a particular round of the two-layer learning algorithm (see Line 4 of \Cref{alg:RAI}). 
We remark that we are unaware of any prior work presenting an FPTAS for a JMS problem with quite general concave rewards. Thus, our results can be of independent interest.  


\smallskip



\noindent\textbf{Numerical Simulations \&  Insights (\Cref{sec:numerical}/Appendix~\ref{apx:numerical-main})} 
We complement our theoretical framework with numerical simulations on synthetic data. Focusing on demographic parity, quota, and budget in the Pandora's box model with two demographic groups, we numerically study both the \emph{short-term} and the \emph{long-term} impacts of imposing socially aware constraints. Concretely, we take the perspective that
the prior available for the quality (or value) of each candidate and its realization upon inspection can be viewed as only a surrogate for the true quality of the candidate which is unobservable in the short run. As such, to measure the short-term impact, we rely on these observable signals. On the other hand, given the opportunity, the true qualities are revealed in the long run. The latter is inspired by the theory of downstream outcomes introduced in \cite{becker2010economics} and is further studied in the literature on the economics of labor discrimination (cf. \cite{canay2020use}). 


We consider scenarios where there is no inherent statistical asymmetry between the two groups in terms of their true qualities (besides the natural heterogeneity in the population). However, the observable signals are systematically biased downward for one group. (This approach is similar to the one taken in \citet{raghavan2020mitigating}.) We investigate the impact of imposing constraints such as demographic party on both the short-term outcomes (measured by biased signals)  and the long-term ones (measured by true qualities) for varying levels of bias. Before proceeding to overview the results of our simulation, let us consider a motivating example. SAT scores serve as an important signal for the long-term success of a student in college admission (measured by, e.g., their 4-year GPA). At the same time, students from disadvantaged backgrounds are known to have lower SAT scores compared to students from privileged backgrounds partly due to lack of proper training.\footnote{A recent study of \cite{Chetty2023Diversifying} uses anonymized admission data from several private and public colleges linked to income tax records and SAT/ACT test scores. They show that one third of the children of the very richest families scored a 1300 or higher on the SAT, while less than 5 percent of middle-class students did, according to the data. Relatively few children in the poorest families scored that high; only one in five took the test at all.} As such, their SAT scores may be an underestimate of their long-term success. 
%, and thus this demographic group may compare unfavorably to students from privileged backgrounds. 
However, if these students are admitted to the college and receive the same training, then they can perform equally well as their peers from privileged backgrounds in the long term. Consequently, imposing constraints such as demographic parity that would lead to admitting more students from this group can even improve long-term outcomes.



% \VMcomment{if we like the above, we can remove the next two parag.  Also, if say all these contexts upfront, we can make S4 shorter. }

% We then consider the scenario where the signals are biased against one of the two demographic groups both in terms of their prior distributions and realized values --- for example, SAT scores for college admissions that could be highly correlated with social class.\footnote{A recent study of \cite{Chetty2023Diversifying} uses anonymized admissions data from several private and public colleges linked to income tax records and SAT/ACT test scores. They show that one-third of the children of the very richest families scored a 1300 or higher on the SAT, while less than 5 percent of middle-class students did, according to the data. Relatively few children in the poorest families scored that high; just one in five took the test at all.} To study the short-term effect, we evaluate and compare the performance of our constrained optimal policy and the unconstrained optimal policy in terms of their expected search utility calculated based on these signals. 

% To study the long-term effects, inspired by the theory of downstream outcomes introduced in \cite{becker2010economics} and studied further in the literature on the economics of labor discrimination (cf. \cite{canay2020use}), we model the unobservable latent ``true quality'' of each candidate. We think of these quantities as the downstream performance of the candidate after given opportunity ---
% for example, the GPA of an admitted college student four years after starting school. We consider the scenario in which there is no inherent statistical asymmetry between the two groups in terms of their true qualities (besides the natural heterogeneity in the population). To measure the long-term effect, we evaluate and compare the performance of our constrained optimal policy and the optimal unconstrained policy by plugging the true qualities into their utility objective. Note that these policies only have access to signals and not the true qualities. See \Cref{sec:numerical} for more details.

Our numerical study delivers several intriguing insights:


\smallskip
\noindent\emph{(i)}~Regarding the short-term effects, our numerical results suggest that even under a moderate amount of bias in the signal and with strong notions of fairness such as demographic parity, ``price of fairness'', that is, 
the relative utilitarian loss due to imposing the constraint}, is small. This is particularly surprising because the selection under the optimal unconstrained policy can be significantly disparate across the two groups. 
This has an important implication: imposing a parity constraint can have substantial egalitarian benefits without drastically harming the short-term utilitarian outcomes (see \Cref{sec:num-short-term}).

\smallskip
\noindent\emph{(ii)}~In terms of long-term effects, our numerical results suggest that imposing socially aware constraints such as demographic parity or quota can even make the search \emph{more efficient} in terms of true unobserved qualities. This also has an important implication: even though the decision maker needs to select based on biased signals, by imposing ex-ante parity constraints, it can calibrate the selections in a way that (partially) corrects the existing bias in signals. By doing so, it can outperform the unconstrained policy that is agnostic to the bias in the signals (see \Cref{sec:num-long-term}). 

\smallskip
\noindent\emph{(iii)}~Finally, 
when the bias in the signals is significantly high, we find that imposing a strict constraint such as demographic parity may not be the most suitable choice, as it causes \emph{unintended inefficiencies} in both short- and long-term outcomes: the decision maker may prefer to keep some part of the capacity \emph{unallocated} to ensure parity. As a result, it is worthwhile considering more lenient variants of demographic parity, e.g., employing quotas with carefully chosen parameters, which can provide representation to minority groups without causing underallocation (see \Cref{sec:numerical-unintended}).


We further study various forms of resource augmentation (e.g., increasing capacity) and constraint adjustments (e.g., tuning the fraction in a quota constraint) and their effects on the relative short-term utility loss and long-term utility gain due to imposing constraints.\footnote{In summary, our results suggest that these simple and small changes can go a long way. In particular, increasing the capacity even a tiny bit can drastically help increase the search utility (with respect to both signals and true qualities). Moreover, by tuning the constraint as mentioned earlier (quota with suitable parameters vs. demographic parity), the effect of increasing capacity on the search utility can be amplified further.} See Appendix~\ref{sec:numerical-parity}, Appendix~\ref{sec:numerical-quota} and Appendix~\ref{sec:numerical-budget} for more discussion. 








 % If the bias is only in the signals received by the decision maker, our numerical results suggest that imposing socially aware constraints such as demographic parity or quota can even help making the search \emph{more efficient with respect to unobserved ground truth values}  so while there seems to be an immediate price of fairness with respect to signals, imposing such constraints can help with long-term outcomes in hiring driven by the true values.~\footnote{Inspired by the concept of ``long-term outcomes'' introduced in \cite{becker2010economics} and studied further in the economic literature on labor discrimination (cf. \cite{canay2020use}), we think of true values as true candidate qualities that are not observable today but can be measured based on long-term outcomes, e.g. the performance of a student at school at the time of graduation; however, the signals are observable today upon inspection, e.g., standardized test scores, but may contain implicit forms of bias.} Furthermore, our results suggest that even in extreme cases where signals are significantly biased (which even under symmetric true values can cause inefficiency; see related discussions in \Cref{sec:numerical}), increasing the capacity  even a tiny bit --- can drastically help with increasing the search utility (with respect to both signals and true values). Moreover, by tuning the constraint as mentioned earlier (quota with suitable parameters vs. demographic parity), the effect of increasing capacity on the search utility can be amplified further.  In a nutshell, our numerical findings suggest that (i) carefully tuning the constraint and (ii) augmenting resources such as capacity can go a long way in terms of imposing diversity while maintaining the search utility. See \Cref{sec:numerical-parity}, \Cref{sec:numerical-quota} and \Cref{sec:numerical-budget} for more discussion. 

 

%Make a connection between the pandora's result this paper \citet{kleinberg2018algorithmic}... disucss the analogy between keeping the within-group orderings... what about inspection? individual distributions?

%In solving the above problem, the decision maker disregards any information about group membership and  implicitly assumes that the distributions are ``comparable'' across groups. However,  it is well documented that in certain contexts there can be a systematic bias toward a demographic groups which makes direct comparison between two groups unfair \citep{raghavan2020mitigating}.  One possible remedy is to impose group-level constraints to ensure a certain  level of parity across the two groups.


\subsection{Further related work}
\label{sec:further-related-work}
\input{tex/related-work}

% \smallskip
% \noindent\textbf{Organization.}
% In \Cref{sec:pandora}, we revisit the Pandora's problem under the fairness notions of parity in selection (\Cref{subsec:FS}) and inspections (\Cref{subsec:IS}), and  present  the optimal fair policies for each case. In \Cref{sec:general}, we present our general setting for Markovian sequential search under a broad class of convex and affine fairness-motivated constraints and present an almost optimal and fair algorithm. 
% %\Cref{sec:delegation} is dedicated to the problem of fairness in  delegated search. 
% \Cref{sec:conclusion} concludes the paper by discussing future directions. 



==> tex/intro-old.tex <==
\section{Introduction}
\label{sec:intro}



Life-changing selection decisions, such as hiring and admission, have long suffered from biases against certain societal groups, leading to a lack of diversity and representation. Despite the continued effort, the progress has been stagnant: the meta-analysis of \citet{quillian2017meta} shows that racial discrimination in hiring has not improved in the last few decades. The rise of algorithmic hiring presented an opportunity to disrupt this pattern and has given rise to a proliferation of 
hiring tools and platforms that aim to mitigate biases and promote equity, diversity, and inclusion \citep{garr2019diversity, raghavan2020mitigating}. 

A key factor contributing to discrimination in algorithmic decision-making is that the ``input'' data -- based upon which decisions are made -- may be biased. 
Take standardized tests, a critical factor in college admission, as an example:  
Students from different socioeconomic classes may have systematically different scores partly due to differences in school quality \citep{sackett2012role, kleinberg2018algorithmic}. 
One school of thought in achieving societally desirable outcomes in the presence of such biases is to incorporate relevant ``fairness'' measures in the underlying decision processes (see the discussion in \citet{kleinberg2018algorithmic}). Subscribing to this school of thought, we study search and selection processes subject to various notions of fairness. Our overarching question is the following:

\begin{displayquote}
{\em How to design optimal and fair search policies for selection problems such as hiring?} 
\end{displayquote}

Toward answering the above question, we first augment the classic model of search known as the {\em Pandora's box} problem \citep{weitzman1979optimal} with certain fairness constraints. In the original model, a decision maker is presented with a set of alternatives (or boxes), and her goal is to select at most one of them; a priori, she only has distributional knowledge about the reward of each box. However, if she inspects a box (at a known cost), she will observe its actual reward and can select it. This model captures the tension between stopping the search (to avoid further inspection costs) vs. continuing it (to find a better alternative). Naturally, the main goal is to find an optimal policy to maximize the net value. Our variant of Pandora's box involves a few modifications: boxes belong to two demographic groups, and the decision maker knows this information upfront. Aware of the implicit biases in distributions or cost disparities across these two groups, the decision maker imposes {\em demographic parity} constraints. We consider two such constraints: (i) parity in the selection, namely equalizing the probability of selecting from each group, and (ii) parity in inspection, i.e., 
equalizing the ex-ante number of inspected alternatives from the two groups. 


We formally define these two settings in Sections \MA{correct references} \ref{subsec:FS} and \ref{subsec:IS}, and for each setting, we characterize the optimal fair policy.\footnote{Throughout this paper, with a slight abuse of terminology, we use the term ``fair'' policy to refer to the policy that satisfies the fairness constraints under consideration.} (See \Cref{alg:FS} and \Cref{thm:FS} for the former and  \Cref{alg:FI} and \Cref{thm:FI} for the latter.) For both settings, we show that the optimal fair policy has a remarkably simple structure: it randomizes between at most two policies, each of which is index-based. Furthermore, both policies rely on the same set of indices and only differ in tie-breaking decisions. More importantly, these indices are simple adjustments to the Gittins index for the original model. (We remind the reader that Pandora's rule given in \citet{weitzman1979optimal} is a Gittins index policy.) 

Generally known to be brittle, it is intriguing that adding these ex-ante constraints does not break the optimality of index-based policies. The reason behind this is the existence of a relaxed Lagrange dual function 
to these constrained problems that can be viewed as an unconstrained Pandora's box problem but for an {\em adjusted instance}. These adjustments have interesting economic interpretations: To achieve parity in the selection, it suffices to uniformly shift the {\em rewards} of all members of a group by a constant 
leaving the inspection costs unchanged (see discussion after \MA{correct references}  \Cref{thm:FS}). On the other hand, to achieve parity in inspection, we must similarly shift the {\em inspection} costs and keep the rewards unchanged. Interestingly, for the case of parity in the selection, such a uniform adjustment in rewards implies that the order of search among members of each group remains the same as in a setting where we conduct searches separately in each group. Preserving {\em within group} order is generally desirable, as discussed in the context of algorithmic fairness. (see \citet{kleinberg2018algorithmic} and references therein). 
Such a property, however, does not always hold for the case of parity in inspection, implying that such a notion of fairness may come at the cost of distorting within group order. (See discussions after Theorems \ref{thm:FS} and \ref{thm:FI} for further elaboration.)
%\VM{follow up todo: let's add two remarks at some point in \Cref{subsec:FS} and \Cref{subsec:IS} to make these points formally.}


While the Pandora's box problem has served as a cornerstone for the study of search problems, realistically,  hiring decisions involve richer search processes. We present one such example below. 

\smallskip
\begin{example}[Multi-stage Search with Rejection]
\label{ex:reject}
Hiring for many jobs involves two stages of inspection. A low-cost one (e.g., 
in the form of a phone interview) and a high-cost one (involving an onsite visit). The first stage only reveals partial information that can be encoded as a pass/fail score. However, the second one reveals the true value of the candidate. At each time, the hiring firm can decide to do the low-cost inspection for a new candidate or the high-cost one for a candidate who has already passed the first stage or stop the search altogether and make an offer -- which can be costly itself -- to a candidate who has undergone both stages. 
The selected candidate may reject the offer with a given probability, wherein the decision-maker can resume the search. 
\end{example}
\smallskip

The above is just one example of a ``stateful'' search process in which the underlying status of a box (e.g., a candidate) can evolve each time the decision-maker interacts with it. As a result, the search process can depend on each box's current observable \emph{state}. This state encodes the box's status and the cost of inspecting it (or the current reward for selecting this box if it is ready to be selected). The stateful nature of these applications gives rise to highly complex policies that may suffer from various types of biases in different stages of the search process or their outcomes. Motivated by this, in \Cref{sec:general}, we study how to incorporate a reasonably \emph{general class of ex-ante fairness constraints} in such settings. Going beyond the basic Pandora's box model and the particular notion of demographic parity,  we model a general Markovian sequential search problem as a \emph{joint Markov scheduling (JMS)} problem -- which has been extensively studied in the literature~\citep{gittins1979bandit,dumitriu2003playing} -- under our general fairness notion.


A Markovian sequential search problem can be captured using JMS by modeling each box as an {\em absorbing} Markov chain (MC) with terminal states. 
Each time the decision maker interacts with a box, the corresponding MC undergoes a stochastic state transition. The selection of a box is encoded by transitioning to a terminal state. Each state is associated with a reward, often negative for non-terminal states (capturing costs) and positive for the terminal ones (encoding potential gain from selection).
\footnote{As we see later in \Cref{sec:optimal-JMS-arbitrary}, for reasons related to incorporating fairness by adjusting the rewards, we need to go beyond this setting and consider problem instances with \emph{arbitrary} positive or negative state rewards.}
The search process entails selecting one of these MCs sequentially until the currently selected MC reaches a terminal state (capturing a final selection). In the base (unconstrained) model, the decision maker's goal is to adaptively select one of these MCs to maximize her expected net value. In \Cref{sec:JMS-setting}, we formally introduce the setting. Further, in Figures \ref{fig:pandora-jms} (resp.  \ref{fig:MC-hiring}), we illustrate the JMS representation for a toy instance of Pandora's box (resp. \Cref{ex:reject}). 

%\VM{my suggestion: switch the order in fig 1 and then also explain Pandora a bit more. There is nice footnote in the next parag. that is currently commented out. I think we can just condense this and put in it the caption?}     



%CFN: To model the utilities, each state is associated with a reward, which is usually assumed to be negative for non-terminal states as a cost should be paid for inspecting an arm, and positive for terminal states  as a value is made from selecting an arm.\footnote{As we see later in \Cref{sec:optimal-JMS-arbitrary}, for reasons related to incorporating fairness by adjusting the rewards, we need to go beyond this setting and consider problem instances with \emph{arbitrary} positive or negative state rewards.} The goal of the decision maker is to adaptively select and interact with these MCs to maximize the total collected rewards until one of the chains reaches a terminal state (and hence be selected).  Importantly, this model also subsumes the Pandora's box model of \cite{weitzman1979optimal} as a special case.\footnote{To see this, for each box $i\in[n]$ consider a Markov reward process with one initial state ``not opened'' with reward $-c_i$, one state for each possible value realization $v_i\in\values_i$ with reward $v_i$ (and state transition probability of $F_i(v_i)$ from the initial state), and one terminal state with reward $0$.} 

Equipped with the JMS framework, we incorporate notions of fairness beyond demographic parity considered in \Cref{sec:pandora}. We allow any arbitrary \emph{affine or convex constraint over the vector of ex-ante outcomes} of the search process. At a high level, for a given policy, we focus on the vector of the expected number of visits for each state of each box, and we impose our constraints on such a vector.  
Our approach is flexible enough to capture various notions of group-level and individual fairness considered in the literature. 
For example, in the spirit of the widely-practiced $4/5$ rule~\citep{raghavan2020mitigating}, the decision maker may aim to approximately equalize the ex-ante rate of selection (or offers) across demographic groups (up to a $4/5$ factor). Further, in contexts such as hiring, advancing in the search process may come with benefits (e.g., gaining experience or visibility) even if the candidate is not selected. Our framework can also capture this by defining a utility function for each box that depends on its ex-ante outcomes. Based on these utilities, the decision maker may want to maintain equity among similar individuals by incorporating non-linear egalitarian welfare measures such as Nash social welfare or minimum utility in her fairness constraints~\citep{kaneko1979nash,dwork2012fairness}. We also formalize our fairness constraints and our general optimal fair problem in \Cref{sec:JMS-setting}.  

In \Cref{sec:RAI}, we present a polynomial time algorithm, called {\em Generalized Randomized Dual-adjusted Index Policy} (G-RDIP), that finds an almost fair and optimal policy. Concretely, given positive constants $\epsilon$ and $\delta$, we find a policy with an objective value within an additive $\epsilon$ factor of the optimal fair solution. It also satisfies all the constraints within an additive factor of $\delta$ (see \Cref{alg:RAI} and \Cref{thm:RAI}). Similar to \Cref{sec:pandora}, an essential building block of our algorithm design is the optimal solution for the base JMS problem. Prior work has shown that JMS admits a Gittins index optimal policy under certain assumptions on the state rewards~\citep{gittins1979bandit,dumitriu2003playing}. In   \Cref{sec:optimal-JMS-arbitrary}, we refine these results to show that the index-based structure of the optimal policy can be preserved even for arbitrary state rewards through a pre-processing step (see \Cref{thm:JMS-optimal-reduction-informal}). 

The above refinement is necessitated by our key observation that, similar to \Cref{sec:pandora}, the Lagrangian relaxation of the optimal fair problem can be viewed as an unconstrained JMS for an adjusted instance. However, with convex constraints, the objective function of the new JMS will no longer be linear in the ex-ante outcome vector. To overcome this challenge, we further relax the  Lagrangian dual function to a linearized version by applying the Fenchel weak duality. (We review the basics of this machinery in  \Cref{sec:convex}.) Taking a game-theoretic view for solving convex optimization and saddle-point problems, we aim to solve the zero-sum game (between the primal and dual players) associated with each of these relaxations. Our algorithm G-RDIP finds an approximate equilibrium strategy for both games using a simple iterative learning algorithm that crucially exploits our problem's structure. We provide an overview of our design in \Cref{sec:RAI}. 
%CEC \VM{should we say more and talk about co-linearity of $\mu$ and $\beta$? I'd say no.}


The resulting algorithm randomizes among polynomially many index-based policies, each of which is an optimal policy for a JMS instance with adjustments based on the dual estimates of a particular round of the learning algorithm (see Line 4 of \Cref{alg:RAI}). We  present an analysis of G-RDIP in \MA{correct references}  \Cref{sec:RAI-analysis} and prove \Cref{thm:RAI}. 
We remark that we are unaware of any prior work presenting an FPTAS for a JMS problem with concave rewards. Thus, our results can be of independent interest.  




%Make a connection between the pandora's result this paper \citet{kleinberg2018algorithmic}... disucss the analogy between keeping the within-group orderings... what about inspection? individual distributions?

%In solving the above problem, the decision maker disregards any information about group membership and  implicitly assumes that the distributions are ``comparable'' across groups. However,  it is well documented that in certain contexts there can be a systematic bias toward a demographic groups which makes direct comparison between two groups unfair \citep{raghavan2020mitigating}.  One possible remedy is to impose group-level constraints to ensure a certain  level of parity across the two groups.
\vspace{-2mm}

\subsection{Further related work}
\label{sec:further-related-work}
\input{tex/related-work}

\smallskip
\noindent\textbf{Organization.}
In \Cref{sec:pandora}, we revisit the Pandora's problem under the fairness notions of parity in selection (\Cref{subsec:FS}) and inspections (\Cref{subsec:IS}), and  present  the optimal fair policies for each case. In \Cref{sec:general}, we present our general setting for Markovian sequential search under a broad class of convex and affine fairness-motivated constraints and present an almost optimal and fair algorithm. 
%\Cref{sec:delegation} is dedicated to the problem of fairness in  delegated search. 
\Cref{sec:conclusion} concludes the paper by discussing future directions. 



==> tex/mreza-discussions-numerical.tex <==
\section{Mohammad Reza's stuff}

\MA{add a couple of biased histograms}


% In the previous sections we have seen how we can find (almost) optimal solution to an algorithmic search problem, where the goal is to maximize the total acquired utility while satisfying rather general multiple affine and convex constraints. As we our target impact is a socially aware search process, in our examples, we pay a particular attention to some fairness/diversity/budget constraints, including, demographic parity, quota, and (scholarship) budget constraints.


First, in \Cref{subsec: simulation-parity-biased}, we consider the demographic parity as our social constraint and study the different aspects of the optimal fair policy as well as the optimal unfair one, under various capacity and Bias Factor values. 

Second, in \Cref{subsec: simulation-parity-groundTruth}, we consider the situation in which the bias factor is due to an ill-accurate (historical) evaluation data that is available for candidates in $\WomanSet$. In fact, these people, given the opportunity, would perform as talented and skilled as candidates in $\ManSet$ in the long run. However, this above-expectation performance will only be realized in future, when both of the fair and unfair optimal algorithms have long made their decisions based on the "ill-judged" biased data. 

Third, in \Cref{subsec: simulation-quota-biased} and \Cref{subsec: simulation-quota-groundTruth} , we consider the quota as our social constraint and study the different aspects of the optimal fair policy as well as the optimal unfair one, under various capacity, Bias Factor, and quota threshold values. 

Lastly, in \Cref{subsec: simulation-budget}, we consider the a scenario where the decision maker is endowed with some exogenous budget that is meant to be only used toward selection from the underprivileged group $\WomanSet$. You can think of this budget as an scholarship budget given to an institution, in order to admit/hire disadvantaged individuals that are otherwise unable to pay the tuition, fees, moving costs, etc. We will explain more on this later on, at the corresponding subsection.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\MA{Discussions start here:}

Discussions:

% %%%%%%%%%%%%% %%%%%%%%%%%%
1- Demo/Quota, Impact of Biased Signals, (ground truth setting):

If signals are low/moderately biased (bias factor $\rho \geq 0.3$), enforcing demographic parity will actually improve the true utility compared to the unconstrained optimal policy - under capacities larger than 1 - by countering the bias to some extent, and resulting in a better selection with regard to the true values. On the other hand, when signals are extremely biased (bias factor $\rho \leq 0.2$), enforcing strict demographic parity can be inefficient as it may eventually result in sub-optimal selections, i.e., not utilizing the decision maker's full capacity for hiring. This can be observed in \Cref{fig:v3_diff_and_CR_fair_unfair}

In cases of extreme signal bias, relaxing the enforcement of demographic parity and opting for quota-based approaches might be more efficient.
Quotas ensure a minimum representation of underrepresented groups without being overly rigid, allowing for more flexibility in candidate selection. To read more about this, we refer to the \Cref{subsec: simulation-quota-groundTruth} and \Cref{fig:v6_diff_CR_fair_unfair}.

Striking the right balance between ensuring diversity (demographic parity or quota) and selecting the most qualified candidates is essential for optimizing the true utility of the selection process. Decision-makers may need to adapt their approach based on the severity of signal bias and the specific context to maximize the efficiency and fairness of the selection process.

In summary, the trade-off between enforcing demographic parity and optimizing true utility becomes critical when dealing with biased signals. Flexibility in approach, such as utilizing quotas in extreme cases, can help maintain fairness while ensuring efficient and effective decision-making.

% %%%%%%%%%%%%% %%%%%%%%%%%%
2,3,4- Demo/Quota, Impact of Biased values:

In the scenarios that bias is low (bias factor $\rho \geq 0.7$), we can observe from \Cref{fig:v1_diff_and_CR_fair_unfair} that the price of fairness is not only very small but also invariant w.r.t. $k$. However, when we look at \Cref{fig:v1_slack_lambda_fair_unfair}, we can see that the optimal unfair policy incurres a considerably large slack in its fairness constraints - except when $\rho=1$ (no bias) - suggesting the phenomena that even though the optimal unconstrained is far from being fair, there might be some almost optimal solutions that can both satisfy our fairness constraint and enjoy a very low price of fairness, and our optimal fair procedure is trying to find the "most fair" one among them.


On the other hand, when dealing with a highly biased prior (bias factor $\rho \leq 0.5$), enforcing a constraint like demographic parity, which aims for a 50-50 balance, might hurt the price of fairness significantly, which only gets worse when $k$ increases. This is because it introduces a new kind of inefficiency by pressuring a socially aware decision maker to refrain from fully utilizing its selection capacity. In these situations, our research suggests that imposing such a strict constraint might not be the most suitable approach, worthwhile considering more lenient variants of demographic parity, e.g., employing quotas with carefully chosen parameters, can provide representation to minority groups without compromising overall efficiency.


% %%%%%%%%%%%%% %%%%%%%%%%%%
5- Comparing the gain through additional budget vs. additional capacity:

\MA{Needs your table from v4.}



% %%%%%%%%%%%%% %%%%%%%%%%%%
6- Dominated capacity for Demo and Quota:

In scenarios that bias is low ($\rho \geq 0.7$), we can observe from \Cref{fig:v1_dominated_capacity} that the required amount of extra capacity in order to surpass the optimal unconstrained (without the extra capacity) is not much, especially if we look at it as the percentage of the original capacity. This amount highly increases as $\rho$ decreases, indicating that for low biased societies, with an small increment on resource/capacity we can go a long way while satisfying our parity constraint, where as in highly biased societies, it requires a significant amount of extra resource/capacity such that we can be as good while satisfying the constraint. This phenomenon, might also be another indicator that in highly biased populations, the decision maker should consider being more flexible, while maintaining a good representation of the underprivileged group, by considering a quota constraint with $\theta<0.5$.

In this regard, if we look at \Cref{fig:v5_dominated_capacity}, the horizontal distances between the curves indicate that with one unit of more capacity (right curve compared to the left curve) how much we can increase the coefficient of the quota, while still achieving the same amount of utility. As shown in these graphs, we can see that this horizontal distance is actually quite large for small $\theta$ and decreases when $\theta$ increase, suggesting the fact that a small increase in capacity can go a long way in satisfying stricter quota constraint, especially when the objective of the decision maker is not high thetas ($\theta<0.3$) for reasons discussed above (on why it should be more flexible compared to the 50-50 rule of demographic parity).














==> tex/prelim.tex <==
\section{Preliminaries}
\label{sec:prelim}

